Simultaneous Contests with Equal Sharing Allocation of Prizes: Computational Complexity and Price of Anarchy

We study a general scenario of simultaneous contests that allocate prizes based on equal sharing: each contest awards its prize to all players who satisfy some contest-specific criterion, and the value of this prize to a winner decreases as the number of winners increases. The players produce outputs for a set of activities, and the winning criteria of the contests are based on these outputs. We consider two variations of the model: (i) players have costs for producing outputs; (ii) players do not have costs but have generalized budget constraints. We observe that these games are exact potential games and hence always have a pure-strategy Nash equilibrium. The price of anarchy is $2$ for the budget model, but can be unbounded for the cost model. Our main results are for the computational complexity of these games. We prove that for general versions of the model exactly or approximately computing a best response is NP-hard. For natural restricted versions where best response is easy to compute, we show that finding a pure-strategy Nash equilibrium is PLS-complete, and finding a mixed-strategy Nash equilibrium is (PPAD$\cap$PLS)-complete. On the other hand, an approximate pure-strategy Nash equilibrium can be found in pseudo-polynomial time. These games are a strict but natural subclass of explicit congestion games, but they still have the same equilibrium hardness results.

==> aaai/best-response.tex <==
\section{Multi-Activity: Hardness of Best-Response}\label{sec:multiActivity}
In this section, we shall prove the hardness results for best-response in the multi-activity models. In particular, we shall prove that even with a single player the optimization problem of finding a best strategy is NP-hard; and therefore, finding an equilibrium is NP-hard. This shows that although the multi-activity model is quite natural and nicely represents practical situations and matches real-world data~\cite{may2014filter}, it is a bit too general. In the next section, we shall study the single-activity cost and budget models.

\begin{theorem}\label{thm:hardBestResp}
In the multi-activity models, both cost and budget, it is NP-hard for a player to optimally play the game.
\end{theorem}
\begin{proof} %[Proof of Theorem~\ref{thm:hardBestResp}]
We provide a reduction from {\sc Set-Cover}. We use the optimization version of the {\sc Set-Cover} problem for the cost model and the decision version of the problem for the budget model.

{\sc Set-Cover}: Let there be a universe $\cU = \{1, 2, \ldots, \hat{m}\}$ and a set of subsets of $\cU$ of size $\hat{k}$, $\cS = \{S_1, S_2, \ldots, S_{\hat{k}}\}$. The optimization problem is to find a smallest set cover: select a subset of $\cS$ of the smallest possible size that covers $\cU$. The decision problem is to tell whether there exists a set cover of size $\kappa \in [\hat{k}]$.

We first focus on the cost model, then we slightly modify the same construction for the budget model.

\textbf{Cost.} We create an instance of the multi-activity cost model with $1$ player, $m = \hat{k} + \hat{m}$ contests, and $k = \hat{k}$ activities. Let us denote the first $\hat{k}$ contests as $M_1 = \{1, \ldots, \hat{k}\}$ and the next $\hat{m}$ contests as $M_2 = \{\hat{k}+1, \ldots, \hat{k}+\hat{m}\}$.
\begin{itemize}
    \item For the first $\hat{k}$ contests, $M_1$, let each contest have a prize of value $(\hat{m} + 1/2)$. Let the weights for these contests be defined as:
    \[
        w_{j,\ell} = \begin{cases} 1,&\text{ for $\ell = j$}\\
        0,&\text{ otherwise}\end{cases}
    \]
    where $j \in M_1$ and $\ell \in K$. Basically, a contest $j \in M_1$ awards a prize of $(\hat{m} + 1/2)$ to the player iff she produces an output of at least $1$ along activity $j$.
    \item For the next $\hat{m}$ contests, $M_2$, let each contest have a prize of value $1$. A contest $(j+\hat{k}) \in M_2$ awards its prize of $1$ to the player iff she produces a total output of $1$ along activities $\{ \ell \mid j \in S_{\ell} \}$. Formally, the weights are:
    \[
        w_{j,\ell} = \begin{cases} 1,&\text{ if $ (j-\hat{k}) \in S_{\ell}$}\\
        0,&\text{ otherwise}\end{cases}
    \]
    where $j \in M_2$ and $\ell \in K$.
    \item The player has a marginal cost of $(\hat{m} + 1)$ for producing output along any of the activities, i.e., $c_{1,\ell} = (\hat{m} + 1)$ for $\ell \in K$.
\end{itemize}

From the construction above, observe that the contests in $M_1$ are much more valuable to the player than the ones in $M_2$: each contest in $M_1$ has a prize of $(\hat{m}+1/2)$, which is more than the total prize for all contests in $M_2$. Note that the player would never produce an output of strictly more than $1$ along any activity because that would contribute to her cost without affecting the prizes she gets. Also, the player would not produce an output of strictly between $0$ and $1$ for any activity. Because, an output of $b_{1,\ell} \in (0,1)$ along an activity $\ell \in K$ cannot help get any prizes from the contests in $M_1$ (these contests need an output of $1$ along individual activities), and for the contests in $M_2$, it may get prizes when accompanied by another output along some $\ell' \in K$ to make a total output of $1$, but the cost for producing this is $(\hat{m}+1)$, which is more than any prize from these contests (which is at most $\hat{m}$). So, the player produces binary outputs (either $0$ or $1$) along the activities, i.e., she selects a subset of activities from $K$ where she produces an output of $1$ each.

Now, considering only the contests in $M_1$, producing an output of $1$ along any activity gets them a prize of $(\hat{m}+1/2)$ from the contests in $M_1$ and a cost of $(\hat{m}+1)$, so overall utility of $(-1/2)$. So, considering only these contests, the player has no incentive to produce any output along any activity. But, each contest in $M_2$ has a prize of $1$ which can offset this cost of $(1/2)$. So, the player would try to produce output along the minimum possible number of activities in a way to get the prize from all the contests in $M_2$, which is exactly the objective in the {\sc Set Cover} optimization problem.

\textbf{Budget.} The construction for the budget model is the same as the cost model, except that the player does not have any cost for producing output along any activity but has a total output budget of $\kappa$.

As argued before, the contests in $M_1$ are much more valuable than the ones in $M_2$, and contests in $M_1$ award prizes only if a player produces an output of $1$ along individual activities; therefore, the player selects $\kappa$ activities and produces an output of $1$ along those. Now, the player would also like to select these $\kappa$ activities in a manner to win as many of the contests in $M_2$, and if possible, all. This is equivalent to solving the {\sc Set Cover} decision problem.
\end{proof}

As proved in the theorem above, best-response is NP-hard in multi-activity games. It is easy to observe that best response is easy in single-activity games: the player selects an activity among the $k$ activities, and then for the selected activity, the player selects the level of output (for which they essentially have to select among at most $m$ output levels, depending upon the minimum criteria to win the contests).

==> aaai/conclusion.tex <==
\section{Future Work}
%In this paper, we studied a practically relevant model of contests and analyzed its properties: existence of equilibria, price of anarchy, and the computational complexity of finding an equilibria.

An important future direction is to find computationally tractable, yet relevant in real-life, special cases of the model. For the multi-activity model, the problem is NP-hard even with a constant number of players, as shown in Section~\ref{sec:multiActivity}. But, in the single-activity model, the problem becomes tractable with a constant number of players: the number of actions for a player is polynomial in the number of activities and contests, we can explicitly construct a polynomial-size normal-form game and find the PNE, which puts the problem in XP. A thorough investigation on fixed-parameter tractability w.r.t. relevant parameters, including the number of contests, activities, and players, and their combinations, is a good research direction. One can also study the complexity of an approximate equilibrium for the models; some PLS-complete problems have polynomial-time algorithms for an approximate PNE, while for others, an approximate PNE is also PLS-complete~\cite{skopalik2008inapproximability}.

Another direction is to apply the three-level model, player--activity--contest, to contests with other types of prize allocation rules rather than the equal-sharing allocation, like rank-based allocation, proportional allocation, etc.; for which one may study properties of the equilibria and the computation complexity. We also believe that there is a lot to explore along computational complexity of simultaneous contests in general.





% \abheek{reduction from an arbitrary congestion games? gap introducing reduction from FLIP?}

% \paul{As we discussed, it may be of interest to find a generalisation to which we can reduce the problem of finding a mixed NE of an explicit congestion game.}

% \paul{Another item: I don't think there's any issue of social welfare, right now, in these games, is that right? The $n$ players spend their budgets of 1 without any cost, and all prizes are awarded. But in a mixed equilibrium, there may be contests that with positive probability, no-one enters.}
% \abheek{Answer to Paul's second question, added a portion about social welfare, Section~\ref{sec:pnepoa}.}

==> aaai/intro.tex <==
\section{Introduction}
Contests are games in which players invest efforts and produce outputs toward winning one or more prizes, where investments of efforts are costly and irreversible, and the prizes are allocated based on the values of outputs. They are prevalent in many areas including sports, rent-seeking, patent races, innovation inducement, labor markets, college admissions, scientific projects, crowdsourcing and other online services.\footnote{See the book by \citet{vojnovic2015contest} for an introduction to and applications of contest theory.}

In this paper, we study a model with the following properties: 
There are $m$ contests, $n$ players, and $k$ activities, and the contests run simultaneously. 
The players participate in the contests by producing outputs along the set of activities. Each player either has a cost for producing output along an activity, where the cost function may vary depending upon the player--activity pair; or a generalized budget constraint, where each player is associated with a feasible set of output vectors that they can produce along those activities. 
The contests have equal sharing allocation of prizes: each contest equally distributes its prize to the players who satisfy a certain success criterion. This criterion is based upon the outputs produced along the activities; different contests may have different values for the activities, and therefore, different success criteria. 
% \begin{enumerate}
%     \item There are $m$ contests, $n$ players, and $k$ activities, and the contests run simultaneously.
%     \item The players participate in the contests by producing outputs along the set of activities. Each player has a generalized budget constraint: a player is associated with a convex set representing the feasible output vectors that they can produce along those activities.
%     \item The contests have equal sharing allocation of prizes: each contest equally distributes its prize among the players who satisfy a certain criteria. This criteria is based upon the outputs produced along the activities, different contests may have different values for the activities. 
% \end{enumerate}
A restricted version of the budget model has previously been studied in the literature, e.g., by \citet{may2014filter} to study competition among social media curators to gain followers, where the curators correspond to the players and the followers to the contests. 

Our model is different from most models studied in the contest theory literature in two main aspects: (i) the contests have equal sharing allocation of prizes; (ii) the players produce output along activities and not directly for contests. 
The equal sharing allocation of prizes approximates situations where the prize is distributed among players who satisfy certain success criteria, e.g., a funding agency may have to distribute its budget among eligible candidates (or allocate its budget randomly among eligible candidates, which leads to equal sharing, in expectation). Another practical situation captured by this prize-structure is when prizes correspond to non-monetary reputation. In many online discussion forums, the members are awarded badges based on their contributions, but the value of a badge for an individual member arguably decreases as it gets awarded to more and more members~\cite{immorlica2015social}. Intuitively, a similar phenomenon may happen to the reputation of any honorable status as it gets awarded to more people.

The choice for the players to produce output along different dimensions is a common real-life occurrence. A researcher has a choice to invest effort along a set of research areas (activities) to acquire funding from various sources (contests). In the problem studied by \citet{may2014filter}, a social media curator has the choice to select the \textit{type} of content depending upon the topic, quality, length, etc. and produce content of that type, which wins them a different (possibly overlapping) set of followers. Similar choices may be available to the members of online forums to earn points and reputation. The player--activity costs or budgets capture the distinct ability of a player to perform well in some activities compared to others.

These contests have the desirable property that a pure-strategy Nash equilibrium (PNE) always exists.
The price of anarchy (PoA) for PNE is $2$ (tight) for the budget model, but can be infinity for the cost model.
These results for a restricted version of the budget model were proved by \citet{may2014filter}, we easily extend it to our budget model; and we prove corresponding results for the cost model.

On the computation side, we show that although a PNE always exists, it may be difficult to reach. If the players can produce output along multiple activities simultaneously,
%(the model of \citet{may2014filter} allows this)
it is NP-hard for a player to even best-respond given the strategies of other players. 
% Best-response remains hard for even one player. 
The NP-hardness result for best-response motivates us to focus on a restricted model, where a player can produce output only along a small (polynomial) number of portfolios of activities. This model still captures salient features of the previous model: the players have the option to select among several portfolios, and where different players may have different costs or budgets for different activities.

This portfolio model can be reduced to a model where a player cannot produce output along multiple activities simultaneously and has to focus on only one activity at a time; we call it the single-activity model.
% In this model, the set of feasible output vectors for a player does not form a convex set, but any game of this type can be reduced to a game where the set of feasible output vectors is convex and still has same equilibrium strategies for the players. 
The same positive results---the existence of PNE and bound on PoA---that hold for the multi-activity model hold for the singe-activity model as well. In the single-activity model, it is easy for the players to best-respond to the strategies of other players, but we get another hardness result: although a PNE always exits, finding it is PLS-complete. And, if we allow mixed-strategy Nash equilibrium (MNE), the problem is complete for the class PPAD$\cap$PLS. 
% A recent paper by \citet{fearnley2021complexity} proved that finding a fixed-point of a smooth $2$-dimensional function $f : [0,1]^2 \rightarrow \bR$ using gradient descent is (PPAD$\cap$PLS)-complete; based on this result, \citet{babichenko2021settling} proved that finding an MNE of an explicit congestion game is also (PPAD$\cap$PLS)-complete. 
Our result adds another natural and practically relevant problem to (PPAD$\cap$PLS)-complete, which includes fixed-point of gradient descent and MNE of explicit congestion games.

% All omitted proofs are provided in the appendix.

\subsection{Related Work}
The paper most closely related to ours is of \citet{may2014filter}. They introduced a budget version of the model to study competition among social media curators to acquire followers. They prove the existence of a PNE by showing equivalence to an exact potential game (see Definition~\ref{def:potentialGames}), and give the PoA bound of $2$. They also do an empirical study and show that the real-life behavior resembles the predictions of the model. The book by \citet{vojnovic2015contest}, Chapter 5 Section 5.5, presents a slightly generalized model with similar results; our budget model generalizes both these budget models. To our knowledge, the work of \citet{may2014filter} is the only paper that studies a three-component player--activity--contest model.

Models of simultaneous contests that do not have activities, rather the players directly produce outputs for individual contests (equivalently, there is a one-to-one mapping between the activities and the contests), have been extensively studied. Cost-based models where the prizes are awarded based on the ranks of players have been studied by \cite{amann2008parallel,archak2009optimal,bapna2010vertically,dipalantino2009crowdsourcing}, including empirical work by \cite{archak2009optimal,dipalantino2009crowdsourcing,lakhani2010topcoder,yang2008crowdsourcing}. Colonel Blotto games, where the players have budget constraints and the prize is awarded to the highest output player for each contest, were introduced by \citet{borel1921analyse}, and have been extensively studied in the literature (e.g., \citet{borel1938application,tukey1949problem,gross1950continuous,blackett1954some,blackett1958pure,bellman1969colonel,shubik1981systems,roberson2006colonel,hart2008discrete,adamo2009blotto,roberson2006colonel,hortala2012pure,washburn2013or}). Simultaneous contests with proportional allocation has been studied by, e.g., \cite{feldman2005price,zhang2005efficiency,palvolgyi2010strategic}.

The complexity class PLS (Polynomial Local Search) and the concepts of PLS-hardness and PLS-completeness, were introduced by \citet{johnson1988easy}. PLS consists of discrete local optimization problems whose solutions are easy to verify (the cost of a given solution can be computed in polynomial time and its local neighborhood can be searched in polynomial time). Similar to NP-hard problems, PLS-hard problems are believed not solvable in polynomial time. Several natural problems, like finding a locally optimal solution of {\sc Max-Cut}, were shown to be PLS-complete by \citet{schaffer1991simple}. The complexity of finding a PNE of an explicit congestion game, which always has a PNE, is also PLS-complete~\cite{fabrikant2004complexity}, from which it follows that better or best response dynamics take an exponential time to converge in the worst case.

The class PPAD (Polynomial Parity Arguments on Directed graph), was introduced by \citet{papadimitriou1994complexity}. Like PLS problems, PPAD problems always have solutions. For PPAD, the existence of a solution is based on a parity argument: in a directed graph of possibly exponential size, where each vertex has at most one predecessor and one successor, which can be returned by a polynomial-time function for any given vertex. Given a source vertex with no predecessor, the task is to find some other degree-1 vertex.
One of the most well-known results of algorithmic game theory, the complexity of finding a (mixed-strategy) Nash equilibrium (MNE) is PPAD-complete~\cite{daskalakis2009complexity,chen2009settling}. 

Recent work has identified the complexity of computing an MNE of an explicit congestion game. The class PPAD$\cap$PLS represents problems that can be solved either by an algorithm that solves PPAD problems or an algorithm that solves PLS problems. 
Finding an MNE of an explicit congestion game is in PPAD$\cap$PLS because it can be done by either finding a PNE (which is also an MNE) using an algorithm for PLS problems or by directly finding an MNE using an algorithm for PPAD problems.
Recently, \citet{fearnley2021complexity} proved that finding a fixed-point of a smooth $2$-dimensional function $f : [0,1]^2 \rightarrow \bR$ using gradient descent is complete for the class PPAD$\cap$PLS; based on this result, \citet{babichenko2021settling} proved that finding an MNE of an explicit congestion game is also (PPAD$\cap$PLS)-complete.
PLS-complete, PPAD-complete, and (PPAD$\cap$PLS)-complete problems are considered to be hard problems with no known polynomial-time algorithms.

==> aaai/pne-and-poa.tex <==
\section{Pure Nash Equilibrium and Price of Anarchy}\label{sec:pnepoa}
\subsection{Existence of a Pure Nash Equilibrium}
\subsubsection{Budget Model}
\citet{may2014filter} proved the existence of a PNE in a slightly restricted version of our multi-activity budget game without explicitly defining a potential function, the same proof can be extended to our model as well. For completeness, we give a proof in the appendix using the potential function given in \eqref{eq:budPotFun} and by showing that the multi-activity budget game is an exact potential game (Definition~\ref{def:potentialGames}).
\begin{theorem}\cite{may2014filter,monderer1996potential}\label{thm:multBudExPot}
A multi-activity budget game is an exact potential game, hence has a pure-strategy Nash equilibrium.
\end{theorem}
Although the feasible set of outputs $\cB_i$ is not convex in the single-activity budget game, Lemma~\ref{thm:sin2mulBudRed} proves that it can be reduced to the convex game, and therefore, it also has a PNE.
\begin{lemma}\label{thm:sin2mulBudRed}
% The model where a player cannot produce output along one activity at a time can be simulated by a model where a player can produce output along multiple activities in a feasible convex set $\cB_i$.
With respect to pure-strategy or mixed-strategy Nash equilibrium, a single-activity budget game is reducible to a multi-activity budget game.
\end{lemma}
We prove the above lemma by showing: given an arbitrary instance of a single-activity budget game, where each player can produce output only along one activity at a time, we construct a multi-activity budget game, where each player w.l.o.g. produces output only along one activity at a time in an equilibrium. Also, the actions and the utilities of the multi-activity game corresponds to the single-activity game. The proof is in the appendix.

\begin{corollary}
A single-activity budget game is an exact potential game and has a pure-strategy Nash equilibrium.
\end{corollary}

\subsubsection{Potential Function} 
\citet{may2014filter} did not explicitly provide a potential function to prove the equivalence of the multi-activity budget game to an exact potential game, but we shall need it for proving the PLS-completeness result later in the paper. (This potential function is also used to provide a proof of Theorem~\ref{thm:multBudExPot} in the appendix.)
\begin{equation}\label{eq:budPotFun}
    \phi(\bb) = \sum_{j \in M} v_j H(n_j(\bb)),
\end{equation}
where $H(p) = \sum_{\ell = 1}^p 1/\ell$ is the harmonic sum. Similarly, let us define a potential function for the cost model to be
\begin{equation}\label{eq:costPotFun}
    \phi(\bb) = \sum_{j \in M} v_j H(n_j(\bb)) - \sum_{i \in N} c_i(\bb_i).
\end{equation}
% We shall use this potential function to prove the existence of PNE, and PLS-completeness of computing it, in the single-activity and multi-activity cost games.

\subsubsection{Cost Model}
\begin{theorem}
The single-activity and multi-activity cost games are exact potential games, hence have pure-strategy Nash equilibria.
\end{theorem}
\begin{proof}
Let player $i$ make a move by changing its strategy from $\bb_i$ to $\bb_i'$, and let $\bb = (\bb_i, \bb_{-i})$ and $\bb' = (\bb_i', \bb_{-i})$ be the corresponding pure-strategy profiles. Let $S \subseteq M$ and $S' \subseteq M$ be the contests that player $i$ wins for strategy profiles $\bb$ and $\bb'$, respectively. For a contest $j \in S \setminus S'$, $n_j(\bb') = n_j(\bb) - 1$, and for a contest $j \in S' \setminus S$, $n_j(\bb') = n_j(\bb) + 1$, and for other contests, $n_j(\bb') = n_j(\bb)$. The change in potential is $\phi(\bb') - \phi(\bb)$
\begin{multline*}
    = \sum_{j \in M} v_j (H(n_j(\bb')) - H(n_j(\bb))) \\
        - \left(  c_{i}(\bb'_{i}) - c_i(\bb_i)  \right) + \sum_{\iota \in N \setminus \{i\}}  \left(  c_{\iota}(\bb'_{\iota}) -  c_{\iota}(\bb_{\iota}) \right)
\end{multline*}
\begin{equation*}
    = \sum_{j \in S' \setminus S} \frac{v_j}{n_j(\bb')} -  c_{i}(\bb'_{i}) - \left( \sum_{j \in S \setminus S'} \frac{v_j}{n_j(\bb)} - c_{i}(\bb_{i}) \right),
\end{equation*}
which is exactly equal to the change in utility of the player $i$. Note that we never used the single- or multi-activity property of the model, so the proof applies to both.
\end{proof}

\subsection{Social Welfare and Price of Anarchy}
As defined in the preliminaries, we assume the social welfare to be the total prize that gets allocated minus the total cost, 
$SW(\bb) = \sum_{j \in M} v_j \b1(n(\bb) > 0) - \sum_{i \in N} c_i(\bb_i)$. For the budget model, the cost term is not present. 
% A loss in welfare occurs if some contests are not able to allocate their prize to any player. 
The price of anarchy is $2$ for the budget model, and this is tight (see Example 5.37 of \citet{vojnovic2015contest}). For the cost model, unfortunately, the price of anarchy can be unbounded.

\subsubsection{Budget Model}
\citet{may2014filter}, for their model of the multi-activity budget game, proved that at least half of the total prize is allocated in any PNE; the same result holds for our general model even if we consider MNE (or even correlated equilibria). The proof uses ideas similar to \citet{may2014filter} to prove that the game is $(1,1)$-smooth~\cite{roughgarden2015intrinsic}, provided in the appendix. As a corollary, using Lemma~\ref{thm:sin2mulBudRed}, the same result holds for single-activity budget games.
\begin{theorem}\label{thm:swBudMul}
The social welfare in any mixed-strategy Nash equilibrium of a multi-activity budget game is at least $1/2$ of the optimum social welfare.
\end{theorem}
\begin{corollary}\label{thm:swBudSin}
The social welfare in any mixed-strategy Nash equilibrium of a single-activity budget game is at least $1/2$ of the optimum social welfare.
\end{corollary}

\subsubsection{Cost Model}
\begin{theorem}\label{thm:swCost}
The social welfare in any pure-strategy Nash equilibrium of a single-activity or multi-activity cost game can be arbitrarily low compared to the optimum social welfare.
\end{theorem}
\begin{proof}
Consider an instance with two players, two activities, and two contests; $n=k=m=2$. Contest $j$ distributes a prize of $1$ to players who produce an output of $1$ along activity $j$, and does not care about output along activity $(3-j)$. Player $i$ has a cost of $(1/2 + \epsilon)$ for producing an output of $1$ along activity $i$, and a cost of $(1-\epsilon)$ for producing an output of $1$ along activity $(3-i)$.

Consider the following PNE: player $i$ is producing an output of $1$ along activity $(3-i)$ and an output of $0$ along activity $i$; therefore, each player has a cost of $(1-\epsilon)$, a prize of $1$, and a utility of $\epsilon$. Notice that this is a PNE because if any player $i$ decides to produce output along activity $i$ (which they are currently not doing), then they will get an additional prize of $1/2$ for a cost of $(1/2 + \epsilon)$, which decreases their utility. The total welfare for this equilibrium is $2 (1 - (1-\epsilon)) = 2\epsilon$.

Consider the socially optimal situation where each player $i$ produces output along activity $i$, the total prize allocation is still $2$, but the total cost is $2(1/2+\epsilon)$, so the total welfare is $(1-2\epsilon)$. Therefore, the price of anarchy is $\frac{1-2\epsilon}{2\epsilon} \rightarrow \infty$ as $\epsilon \rightarrow 0$.
\end{proof}

Finally, suppose we consider an alternative definition of social welfare that ignores the players' costs and is based only on the prizes awarded (so, is similar to the budget case). In this version, a simple example shows that the price of anarchy is still unbounded. Consider an instance with one player and two contests (and two corresponding activities), the player can win the first contest with a prize of $\epsilon$ with a cost of $\epsilon/2$ but can win the second contest with a prize of $1$ with a cost of $1$. The player only wins the first contest. The price of anarchy is $1/\epsilon \rightarrow \infty$ as $\epsilon \rightarrow 0$.


==> aaai/ppad-pls.tex <==
\section{Single-Activity: (PPAD$\cap$PLS)-Completeness}
% In the previous section, we saw that it is NP-hard for the players to best-respond to the strategies of other players, and so it is NP-hard to find a PNE for the multi-activity cost and budget games. 
In this section, we focus our attention on single-activity games and show that for both cost and budget models, it is PLS-complete to find a PNE and (PPAD$\cap$PLS)-complete to find an MNE. Note that the set of MNEs of a game is a super-set of the set of PNEs, so finding an MNE is at least as easy as finding a PNE.
%(This PLS-completeness result can be extended to the multi-activity setup, but for that, we already have a stronger NP-hardness result.)

\begin{theorem}\label{thm:ppadPls}
In the single-activity models, both cost and budget, it is (PPAD$\cap$PLS)-complete to find a mixed-strategy Nash equilibrium. 
\end{theorem}
A recent paper by \citet{fearnley2021complexity} proved the interesting result that finding a fixed-point of a $2$-dimensional smooth function ($f : [0,1]^2 \rightarrow \bR$) given by a circuit of addition and multiplication operators using gradient descent, {\sc 2D-GD-FixedPoint}, is complete for the class PPAD$\cap$PLS. Based on this result, \citet{babichenko2021settling} proved that the problem of computing an MNE of an explicit congestion game, {\sc ExpCong}, is also complete for PPAD$\cap$PLS. \citet{babichenko2021settling} do this by first reducing {\sc 2D-GD-FixedPoint} to identical interest 5-polytensor games, {\sc 5-Polytensor}, and then {\sc 5-Polytensor} to {\sc ExpCong}. In our proof for Theorem~\ref{thm:ppadPls}, we reduce {\sc 5-Polytensor} to the single-activity game, proving the required result.

Before moving to the proof, let us define identical interest polytensor games, {\sc $\kappa$-Polytensor}. Polytensor games are a generalization of the better known polymatrix games, {\sc Polymatrix}; {\sc Polymatrix} = {\sc $2$-Polytensor}.
\begin{definition}[{\sc Polymatrix}: Identical Interest Polymatrix Game]
There are $n$ players. Player $i$ chooses from a finite set of actions $A_i$. The utility of player $i$ for action profile $(a_i, \ba_{-i}) = \ba = (a_j)_{j \in [n]} \in \times_{j \in [n]} A_j$ is given by $u_i(\ba) = \sum_{j \in [n], j \neq i} u_{i,j}(a_i, a_j)$, where $u_{i,j} : A_i \times A_j \rightarrow R_+$. The players have identical interest, i.e., $u_{i,j} = u_{j,i}$.
\end{definition}
The definition of {\sc $\kappa$-Polytensor} is similar to {\sc Polymatrix}, instead of $u_{i,j}$ we have $u_S$ where $S \subseteq [n], |S| = \kappa$.
\begin{definition}[{\sc $\kappa$-Polytensor}: Identical Interest $\kappa$-Polytensor Game]\label{def:polytensor}
There are $n$ players. Player $i$ chooses from a finite set of actions $A_i$. 
The utility of player $i$ for action profile $\ba = (a_j)_{j \in [n]} \in \times_{j \in [n]} A_j$ is given by $u_i(\ba) = \sum_{S \subseteq [n], i \in S, |S| = \kappa} u_S(\ba_S)$, where $\ba_S = (a_j)_{j \in S}$ is the action profile of the players in $S$ and $u_S : \times_{j \in S} A_j \rightarrow R_+$.
\end{definition}
When the number of actions for each player, $|A_i|$, is bounded by $m$, note that the representation size of a {\sc $\kappa$-Polytensor} game is $O(n^{\kappa}m^{\kappa})$. In particular, if $\kappa$ is a constant and
$m = poly(n)$, then {\sc $\kappa$-Polytensor} games admit a succinct representation.

\begin{proof}[Proof of Theorem~\ref{thm:ppadPls}]
Let us first focus on the single-activity budget model, towards the end we shall extend this to the cost model. Below, we provide a reduction from {\sc $3$-Polytensor} for a cleaner presentation of the main steps. Similar steps with more calculations apply to {\sc $5$-Polytensor}, provided in the appendix.

\textbf{Budget.} Take an arbitrary instance of {\sc $3$-Polytensor} with $n$ players; we shall use the same notation as Definition~\ref{def:polytensor}. We construct a single-activity game with $n$ players, $\sum_{i \in [n]} |A_i|$ activities, and a polynomial number of contests to be defined later.

The $\sum_{i \in [n]} |A_i|$ activities have a one-to-one association with the actions of the players. The activities are partitioned into $n$ subsets; the $i$-th subset has size $|A_i|$ and is associated with player $i$; we identify these activities by $A_i$. Player $i$ has a budget of $1$ that they can use to produce output along any activity from $A_i$, but they have $0$ budget for the activities in $A_j$ for $j \neq i$. Effectively, as we are in a single-activity model, player $i$ selects an activity from the activities in $A_i$ and produces an output of $1$ along it. Note that the players have disjoint sets of activities for which they can produce outputs.

All the contests we construct are associated with exactly three players and at most three activities. We shall denote a contest by $\cC_{i,j,k}(A)$, where
\begin{itemize}
    \item $i$, $j$, and $k$ are the three distinct players based on whose utility function in the polytensor game, $u_{i,j,k}$, we shall specify the prize of contest $\cC_{i,j,k}(A)$;
    \item the contest $\cC_{i,j,k}(A)$ awards its prize to any player who produces an output of at least $1$ along the activities in $A$;
    \item the activities in $A$ are from $A_i \cup A_j \cup A_k$ with $|A| \le 3$ and $ |A \cap A_{\ell}| \le 1$ for $\ell \in \{i,j,k\}$.
\end{itemize}
We shall call a contest $\cC_{i,j,k}(A)$ a Type-$\ell$ contest if $|A| = \ell$.

Let us focus on a fixed set of three players $\{i,j,k\}$. We create contests to exactly replicate the utility that these players get from $u_{i,j,k}$. If we can do this, then repeating the same process for every set of three players, we will replicate the entire {\sc $3$-Polytensor} game. The utility that player $i$ gets from $u_{i,j,k}$ is $u_{i,j,k}(a_i,a_j,a_k)$, where the $a_i,a_j,a_k$ are the actions of the three players.
We have the following contests:

% \begin{enumerate}
    % \item 
\textbf{Type-3 Contests.} Let us add the contest $\cC_{i,j,k}(a_i,a_j,a_k)$ with prize $v_{i,j,k}(a_i,a_j,a_k)$ for every $(a_i,a_j,a_k) \in A_i \times A_j \times A_k$. We shall specify the $v_{i,j,k}(a_i,a_j,a_k)$ values based on $u_{i,j,k}(a_i,a_j,a_k)$ values, later. Contest $\cC_{i,j,k}(a_i,a_j,a_k)$ distributes a prize of $v_{i,j,k}(a_i,a_j,a_k)$ to players who produce output along the activities $a_i$, $a_j$, or $a_k$. 
    
Say the players $i,j,k$ play the actions $a_i^*, a_j^*, a_k^*$. 
% Let $A_j^- = A_j \setminus \{a_j^*\}$; and for $T \subseteq S$, let $A_T^- = \times_{j \in T} A_j^-$. 
The total prize that player $i$ gets from the contests we added is:
\begin{align}\label{eq:ppadPls:1}
    &\frac{1}{3}{v_{i,j,k}(a_i^*,a_j^*,a_k^*)}
    + \sum_{a_j \neq a_j^*} \frac{1}{2}{v_{i,j,k}(a_i^*,a_j,a_k^*)} \nonumber \\
% \end{align*}
% \begin{align*}
    & + \sum_{a_k \neq a_k^*} \frac{1}{2}{v_{i,j,k}(a_i^*,a_j^*,a_k)}
    + \sum_{\substack{a_j \neq a_j^* \\ a_k \neq a_k^*}} v_{i,j,k}(a_i^*,a_j,a_k).
\end{align}
In the above expression, the first term is for the prize that $i$ shares with $j$ and $k$, the second term is for the prizes that $i$ share with only $k$ but not $j$, similarly, the third term is for the prizes that $i$ shares only with $j$ but not $k$, and the fourth term is for the prizes it does not share with $j$ or $k$. 

In the above expression, the first term $\frac{1}{3}{v_{i,j,k}(a_i^*,a_j^*,a_k^*)}$ resembles the utility  that the players get in the polytensor game, $u_{i,j,k}(a_i^*,a_j^*,a_k^*)$. If we were to set $v_{i,j,k}(a_i^*,a_j^*,a_k^*) = 3 u_{i,j,k}(a_i^*,a_j^*,a_k^*)$, then it will exactly be equal. But, unless we take care of the additional terms in the expression, we are not done. We shall add Type-1 and Type-2 contests to cancel the additional terms.

The expression in \eqref{eq:ppadPls:1} can be rewritten as
\begin{align*}
    &\sum_{a_j \in A_j, a_k \in A_k} v_{i,j,k}(a_i^*,a_j,a_k) - \sum_{a_j \neq a_j^*} \frac{1}{2}{v_{i,j,k}(a_i^*,a_j,a_k^*)} \nonumber \\
    &- \sum_{a_k \neq a_k^*} \frac{1}{2}{v_{i,j,k}(a_i^*,a_j^*,a_k)}
    -\frac{2}{3}{v_{i,j,k}(a_i^*,a_j^*,a_k^*)}.
\end{align*}

\textbf{Type-1 Contests.} Let us add contest $\cC_{i,j,k}(a_i')$ with prize $\sum_{a_i \neq a_i', a_j \in A_j, a_k \in A_k} v_{i,j,k}(a_i,a_j,a_k)$ for every $a_i' \in A_i$. This contest $\cC_{i,j,k}(a_i')$ awards its prize to any player who produces output along activity $a_i'$ (effectively it awards the prize to player $i$ if they produce output along $a_i'$, because no other player can produce output along $a_i'$). Similarly, we add the contests $\cC_{i,j,k}(a_j')$ and $\cC_{i,j,k}(a_k')$ for $a_j' \in A_j$ and $a_k' \in A_k$, respectively. The total prize that player $i$ gets from Type-1 and Type-3 contests is
\begin{align*}
    &\sum_{a_i,a_j,a_k} v_{i,j,k}(a_i,a_j,a_k) - \sum_{a_j \neq a_j^*} \frac{1}{2}{v_{i,j,k}(a_i^*,a_j,a_k^*)} \nonumber \\
    &- \sum_{a_k \neq a_k^*} \frac{1}{2}{v_{i,j,k}(a_i^*,a_j^*,a_k)}
    -\frac{2}{3}{v_{i,j,k}(a_i^*,a_j^*,a_k^*)}.
\end{align*}
As $\sum_{a_i,a_j,a_k} v_{i,j,k}(a_i,a_j,a_k)$ does not depend upon the action $a_i^*$ selected by $i$, the utility of player $i$ is effectively
\begin{multline*}
    - \sum_{a_j \neq a_j^*} \frac{1}{2}{v_{i,j,k}(a_i^*,a_j,a_k^*)} \\
    - \sum_{a_k \neq a_k^*} \frac{1}{2}{v_{i,j,k}(a_i^*,a_j^*,a_k)} -\frac{2}{3}{v_{i,j,k}(a_i^*,a_j^*,a_k^*)}.
\end{multline*}

\textbf{Type-2 Contests.} Let us add a contest named $\cC_{i,j,k}(a_i', a_j')$ with prize $\sum_{a_k \in A_k} \frac{1}{2}{v_{i,j,k}(a_i',a_j',a_k)}$ for every $a_i' \in A_i$ and $a_j' \in A_j$. This contest $\cC_{i,j,k}(a_i', a_j')$ awards its prize to players who produce output along activity $a_i'$ or $a_j'$. In a similar manner, we add contests corresponding to the actions of the other $5$ possible combinations of players among the three players $i,j,k$, like $\cC_{i,j,k}(a_i', a_k')$ for $a_i' \in A_i$ and $a_k' \in A_k$, and so on. The net utility that player $i$ gets from Type-1, Type-2 and Type-3 contests is
\begin{equation*}
    \frac{1}{3}{v_{i,j,k}(a_i^*,a_j^*,a_k^*)}.
\end{equation*}
We set $v_{i,j,k}(a_i,a_j,a_k) = 3 u_{i,j,k}(a_i,a_j,a_k)$ for every $(a_i, a_j, a_k) \in A_i \times A_j \times A_k$, and we are done.

\textbf{Cost.} It is easy to adapt the above proof to the single-activity cost model. All the players, contests, and activities are the same, we just need to replace the budgets with costs. In the proof above, we used the budgets to make sure that player $i$ can produce output only along activities in $A_i$. We can achieve that same for the cost model: for player $i$, set a very low cost for the activities in $A_i$ and very high cost for the activities in $A_j$, $j \neq i$, such that player $i$ always wants to produce output along the activities in $A_i$ and never along the activities not in $A_i$.
\end{proof}

In the previous theorem, we analyzed the complexity of computing an MNE. As we have shown earlier, single-activity cost and budget games always have a PNE, and therefore, it is relevant to know the complexity of computing a PNE. 
% Note that computing a PNE is at least as hard as computing an MNE, because a PNE is also an MNE. 
In the next theorem, we prove that computing a PNE is PLS-complete, and this is true even if all the players are identical. In the proof, we reduce {\sc Max-Cut} to the problem of finding a PNE in a particular class of single-activity games with identical players. For this class of single-activity games, finding an MNE is easy, which highlights that the class of single-activity games where PNE is hard (PLS-complete) to compute is strictly larger than the class of single-activity games where MNE is hard (PPAD$\cap$PLS-complete) to compute. The proof is provided in the appendix.
\begin{theorem}\label{thm:plsCompleteness}
In the single-activity models, both cost and budget, it is PLS-complete to find a pure-strategy Nash equilibrium. The result holds even if every player is identical.
\end{theorem}
A direct corollary of this PLS-completeness result is that better/best-response dynamics takes an exponential number of steps to converge for some instances of the problem.

% A corollary of the PLS-completeness result is that for some instances of the game, better/best-response dynamics takes an exponential number of steps to converge to a PNE. This leads to a natural question: if we assume that a player only makes a move if it increases their utility by at least $\epsilon$, for some constant $\epsilon > 0$, does this process converge to an $\epsilon$-PNE in steps polynomial in $1/\epsilon$ and size of the problem? The answer to this question is negative for exact potential games in general~\cite{skopalik2008inapproximability}. Note that all PLS-complete problems have fully polynomial time approximation schemes (FPTAS) with respect to the potential function~\cite{orlin2004approximate}, but approximation of the potential doesn't imply approximation of each player's utility, there may be a player who can make a move to significantly increase their utility as shown by~\cite{skopalik2008inapproximability}.

==> aaai/prelim.tex <==
\section{Model and Preliminaries}\label{sec:prelim}
Consider a set of $n$ players, $N$, who simultaneously produce output along $k$ activities, $K$, and let there be $m$ contests, $M$, that award the prizes to the players based on their outputs. The contests may have different prizes and may value the activities differently.
Typically, a player's output along some activity may make various contributions to their ability to win different contests.
%Note that this model generalizes a model where the number of activities is equal to the number of contests and there is a one-to-one mapping between the contests and the activities: contest $j$ allocates its prize based only on the players' outputs along activity $j$.

We study two types of model: one, where the players have output production costs; and the other, where the players have generalized output budgets. Player $i \in N$ chooses an output vector $\bb_i = (b_{i,\ell})_{\ell \in K} \in \bR_+^k$ (we shall assume throughout the paper that $\bR_+$ includes $0$).
\begin{itemize}
    \item \textbf{Cost.} Player $i$ incurs a cost of $c_i(\bb_i)$ for producing $\bb_i$, where $c_i : \bR_+^k \rightarrow \bR_+$ is a non-decreasing cost function with $c_i(\bm{0}) = 0$. We shall prove our computational hardness and unbounded PoA results for a simpler model with linear cost functions, where $c_i(\bb_i) = \sum_{\ell \in K} c_{i,\ell} b_{i,\ell}$, but the existence of PNE shall hold for the general model.
    \item \textbf{Budget.} The player does not incur any cost for the output vector $\bb_i$, but $\bb_i$ is restricted to be in a set $\cB_i \subseteq \bR_+^k$. In this model too, the positive results hold for general $\cB_i$, but the negative results hold for a simple model where the players are identical and with a budget of $1$ that can be split amongst the activities. 
\end{itemize}
Let $\bb = (\bb_i)_{i \in N} = (b_{i,\ell})_{i \in N, \ell \in K}$. A contest $j \in M$ equally distributes the prize of $v_j > 0$ to all players in the set $N_j(\bb)$ defined as
\[ 
    N_j(\bb) = \{ i \mid f_j(\bb_i) \ge 1 \},
\]
where $f_j(\bb_i) : \bR_+^k \rightarrow \bR_+$ is an increasing function with $f_j(\bm{0}) = 0$. Let $n_j(\bb) = |N_j(\bb)|$. Again, we shall prove the negative results for a simpler model where $f_j$ is a linear function given as $f_j(\bb_i) = \sum_{\ell \in K} w_{j,\ell} b_{i,\ell}$ where $w_{j,\ell} \in \bR_+$, but the results of Section~\ref{sec:pnepoa} related to the existence of PNE and low PoA hold for general $f_j$.

The utility of a player $i$ in the cost model and the budget model are, respectively,
\begin{align*}
    u_i(\bb) &= \sum_{j \in M} \frac{v_j}{n_j(\bb)} \b1\{i \in N_j(\bb)\} - c_i(\bb_i),\\
    u_i(\bb) &= \sum_{j \in M} \frac{v_j}{n_j(\bb)} \b1\{i \in N_j(\bb)\},
\end{align*}
where $\b1\{\ldots\}$ is the indicator function.

\citet{may2014filter} study the budget model and assume that the set $\cB_i$ of feasible output vectors for player $i$ is convex; we call this the \textit{multi-activity} budget model.\footnote{The model presented in \citet{vojnovic2015contest} has $N_j(\bb) = \{ i \mid \sum_{\ell \in K} f_{j,\ell}(b_{i,\ell}) \ge 1 \}$, where $f_{j,\ell} : \bR_+ \rightarrow \bR_+$ is an increasing function with $f_{j,\ell}(0) = 0$. 
% This model generalizes our model, and therefore, our hardness results also hold for this model. Similarly, the positive results for the existence of PNE and the upper-bound for PoA for this model carries over to our model. 
\citet{may2014filter} study a similar model.
% , with similar results and techniques.
}
In this model, where a player can produce output along multiple activities simultaneously, we shall prove that it is NP-hard for a player to best-respond to the strategies of other players. This implies hardness for finding an equilibrium. We also prove a similar result for the multi-activity cost model.

Noting the hardness result, we consider a restricted setup where the players can produce output along a set of portfolios of activities. A player selects a portfolio $p$ from the set of portfolios $\cP_i \subset \bR_+^k$ and produces output proportional to $p$. We assume that the set of portfolios is finite and of polynomial size. 

This portfolio model can easily be reduced to a model where a player $i$ can produce output along only one activity, where an activity in this model corresponds to a portfolio in the previous model; we call this the \textit{single-activity} model. In the single-activity budget model, $\cB_i$ is associated with a vector $\bar{\bb}_i \in \bR_+^k$ of upper-limits; for any $b_i \in \cB_i$, there is an activity $\ell \in K$ such that $0 \le b_{i,\ell} \le \bar{b}_{i,\ell}$ and $b_{i,t} = 0$ for all $t \neq \ell$. Although the feasible set of outputs $\cB_i$ is not convex in the single-activity budget model, in Lemma~\ref{thm:sin2mulBudRed}, we shall prove that it can be reduced to the multi-activity budget model, and therefore, all positive results for the multi-activity budget model apply to this model. We shall also prove similar positive results for the cost model, both single-activity and multi-activity.
% \abheek{We can directly prove the positive results for the models also, then we will not need Theorem~\ref{thm:single2convexReduction}.}
For the single-activity models, both budget and cost, best-response is easy for a player. But, here we will prove a PLS-completeness result for finding a PNE and (PPAD$\cap$PLS)-completeness result for finding an MNE.

% A specific instantiation of this game, where the set of strategies $\cB_i$ are equal and of a particular form for all players $i \in N$, was used by \citet{may2014filter} to study information sharing in social media platforms.\footnote{They also have a player-specific quality: if a player $i$ is in $N_j(\bb)$, then contest $j$ awards (a share of) the prize with probability equal to $i$'s quality. The same results and techniques apply to this model.} They proved that this game is an \textit{exact potential game} (Definition~\ref{def:potentialGames}) and therefore has a pure strategy Nash equilibrium (PNE). They also proved that the price of anarchy (PoA) of the game is at most $2$. The generalized form of the game, as presented above, was given in \cite{vojnovic2015contest}, which also proves that the results---existence of PNE (Theorem~\ref{thm:eqShr1}) and PoA at most $2$ (Theorem~\ref{thm:eqShr2})---hold for the general formulation of the game.

\begin{definition}[Exact Potential Games]\label{def:potentialGames}\cite{monderer1996potential}
A normal form game is an exact potential game if there exists a potential function $\phi$ such that
\[ u_i(b_i', \bb_{-i}) - u_i(b_i, \bb_{-i}) = \phi(b_i', \bb_{-i}) - \phi(b_i, \bb_{-i}), \]
for any player $i$, any two strategies $b_i$ and $b_i'$ for player $i$, and any strategy profile $\bb_{-i}$ for other players, where $u_i$ denotes the utility function of player $i$. 
\end{definition}
Potential games always have a pure-strategy Nash equilibrium~\cite{monderer1996potential}.

\paragraph{Social Welfare.}
The social welfare is the sum of utilities of the players; we do not weight players differently based on their budgets or costs. For the budget models, the social welfare is equal to the total prize that gets allocated: 
\begin{multline*}
    SW(\bb) = \sum_{i \in N} u_i(\bb) = \sum_{i \in N} \sum_{j \in M} \frac{v_j}{n_j(\bb)} \b1\{i \in N_j(\bb)\} \\
        = \sum_{j \in M} v_j \b1\{n(\bb) > 0\}.
\end{multline*}
A loss in welfare occurs if some contests are not able to allocate their prize to any player. Similarly, for the cost models, the social welfare is
\begin{multline*}
    SW(\bb) = \sum_{i \in N} \left( \sum_{j \in M} v_j \b1\{i \in N_j(\bb)\} - c_i(\bb_i) \right) \\
        = \sum_{j \in M} v_j \b1\{n(\bb) > 0\} - \sum_{i \in N} c_i(\bb_i).
\end{multline*}

==> ec/best-response.tex <==
\section{Multi-Activity: Hardness of Best-Response}\label{sec:multiActivity}
In this section, we focus on a restricted model: each contest uses a linear criterion, and the budget constraint or the cost function of each player is also linear. We call this model the {\em linear multi-activity model}. Formally, for an output profile $\bb = (\bb_i)_{i \in N} = (b_{i,\ell})_{i \in N, \ell \in K}$, the winners of contest $j$ are
\[
    N_j(\bb) = \{ i \mid \sum_{\ell \in K} w_{j,\ell} b_{i,\ell} \ge 1 \},
\]
where $w_{j,\ell} \in \bR_{\ge 0}$ is a non-negative weight that contest $j$ has for activity $\ell$. 
Similarly, the linear budget constraint of a player $i$ is of the form $\sum_{\ell \in K} \beta_{i, \ell} b_{i, \ell} \le 1$, where $\beta_{i,\ell} \in \bR_{> 0}$. Likewise, a linear cost function for player $i$ is of the form $\sum_{\ell \in K} c_{i,\ell} b_{i, \ell}$, where $c_{i,\ell} \in \bR_{> 0}$.

We also impose another constraint: we assume that for each contest its total prize is fixed. That is, each contest $j \in M$ is associated with a total prize $V_j$, and if there are $\ell$ winners, each winner gets a prize $V_j / \ell$.

We study the computational complexity of best-response in this linear multi-activity model. Observe that it suffices to consider this problem for $n=1$. Indeed, consider a player $i\in N$. If there are $\ell$ winners other than $i$ for a given contest $j$, then $i$ gets a prize of $v_j(\ell+1) = V_j/(\ell+1)$ from this contest if she satisfies this contest's criteria, and $0$ otherwise. By scaling the values of all contests appropriately, we reduce $i$'s optimization problem to one where $i$ is the only player in the game.

In the next theorem, we prove that finding a best-response is NP-hard. 
%which implies NP-hardness for finding an equilibrium in these games. 
%EE: one does not imply the other
This indicates that, although the multi-activity model is quite natural and nicely represents practical situations and matches real-world data~\cite{may2014filter}, it may be somewhat too general. 
% In the next section, we shall study the single-activity cost and budget models.

\begin{theorem}\label{thm:hardBestResp}
In the linear multi-activity model, 
the problem of deciding if a player
has a strategy that guarantees her a utility of at least $U$ is {\em NP}-hard (and hence computing a best response is {\em NP}-hard). This holds both for the cost model and for the budget model.
\end{theorem}
\begin{proof} %[Proof of Theorem~\ref{thm:hardBestResp}]
We provide a reduction from {\sc Set Cover}. 

{\sc Set Cover}: An instance of this problem is given by a universe $\cU = \{1, 2, \ldots, \hat{m}\}$, a set $\cS = \{S_1, S_2, \ldots, S_{\hat{k}}\}$, where each $S_j$ is a subset of $\cU$, and a positive integer $\kappa \in [\hat{k}]$. This is a yes-instance if $\cU$ admits a set cover of size $\kappa$, i.e., a collection of sets $\cS'\subseteq \cS$ 
with $|\cS'|\le \kappa$ such that
$\cup_{S_j\in \cS'}=\cU$.
We can assume without loss of generality that 
$\cup_{S_j\in \cS}=\cU$ (as otherwise we obviously have a no-instance) and that $\kappa<\hat{m}$
(as otherwise we obviously have a yes-instance).

We first focus on the cost model. Then we slightly modify the same construction for the budget model.

\textbf{Cost.} We create an instance of the multi-activity cost model with $1$ player, $m = \hat{k} + \hat{m}$ contests, and a set of $k=\hat{k}$ activities $K$. We split the contests into two groups of size $\hat{k}$ and $\hat{m}$, respectively:  $M_1 = \{1, \ldots, \hat{k}\}$ and $M_2 = \{\hat{k}+1, \ldots, \hat{k}+\hat{m}\}$.
\begin{itemize}
    \item Each contest in $M_1$ has a prize of value $(\hat{m} + 1/2)$. Let the weights for these contests be defined as:
    \[
        w_{j,\ell} = \begin{cases} 1,&\text{ for $\ell = j$}\\
        0,&\text{ otherwise}\end{cases}
    \]
    where $j \in M_1$ and $\ell \in K$. That is, a contest $j \in M_1$ awards a prize of $(\hat{m} + 1/2)$ to the player as long as she produces an output of at least $1$ along activity $j$.
    \item Each contest in $M_2$ has a prize of value $1$. To receive the prize of contest $(j+\hat{k}) \in M_2$, the player needs to produce a total output of $1$ along activities $\{ \ell \mid j \in S_{\ell} \}$. Formally, the weights are:
    \[
        w_{j,\ell} = \begin{cases} 1,&\text{ if $ (j-\hat{k}) \in S_{\ell}$}\\
        0,&\text{ otherwise}\end{cases}
    \]
    where $j \in M_2$ and $\ell \in K$.
    \item The player has a marginal cost of $(\hat{m} + 1)$ for producing output along any of the activities, i.e., $c_{1,\ell} = (\hat{m} + 1)$ for $\ell \in K$.
\end{itemize}
We set $U=\hat{m}-\kappa/2$.

Observe that the contests in $M_1$ are much more valuable to the player than the ones in $M_2$: each contest in $M_1$ has a prize of $(\hat{m}+1/2)$, which is more than the total prize of all contests in $M_2$.
Note that it is suboptimal for the player to produce an output that is strictly more than $1$ along any activity: this would contribute to her cost without affecting the prizes she gets. Also, it is suboptimal for a player to produce an output that is strictly between $0$ and $1$ for any activity. Indeed, let 
$K'=\{\ell\in K\mid 0<b_{1, \ell}<1\}$, and set
$\beta=\sum_{\ell\in K}b_{1, \ell}$. Suppose for the sake of contradiction that $K'\neq\emptyset$. The activities in $K'$ do not help the player to win contests in $M_1$. If $\beta< 1$, they do not help the player to win contests in $M_2$ either, so the player can improve her utility by 
setting $b_{1, \ell}=0$ for each $\ell\in K'$.
If $\beta\ge 1$, these efforts may contribute towards winning contests in $M_2$, whose total prize value is $\hat{m}$, but then they incur a cost of at least $\beta\cdot(\hat{m}+1)\ge (\hat{m}+1)$, so again the player can improve her utility by 
setting $b_{1, \ell}=0$ for each $\ell\in K'$.
 Hence, when playing a best response, the player produces binary outputs (either $0$ or $1$) along each activity. In other words, she selects a subset of activities from $K$ and produces an output of $1$ for each.

Now, suppose we started with a yes-instance of {\sc Set Cover}. We can assume without loss of generality that there is a cover of size exactly $\kappa$. By picking the activities that correspond to the sets in the cover, the player incurs a cost of $\kappa(\hat{m}+1)$. She also derives a total utility of $\kappa(\hat{m}+1/2)$
from contests in $M_1$ (as she wins $\kappa$ of these contests) and a total
utility of $\hat{m}$ from contests in $M_2$ (as she wins all of them).
Thus, her total utility is $\hat{m}-\kappa/2$.

Conversely, suppose the player has a strategy $A$ whose total utility is at least $\hat{m}-\kappa/2$. We have argued that in a best response the player's outputs are $0$ or $1$ for each activity, so we can assume that this is the case for $A$. Let $\cS'$ be the collection of subsets that correspond to activities for which the player's output is $1$.
If $\cS'$ does not form a set cover, let $i$ be
some element not covered by $\cS'$, and let $S_j$ be some set that covers $i$. The player's output along activity $j$ is $0$. Increasing it to $1$
results in her winning the contest $j$ as well as the contest $\hat{k}+i$, for a total prize of 
$\hat{m}+1/2+1$ and a total cost of $\hat{m}+1$, 
thereby increasing her utility. Thus, we can assume that the set of activities for which the player's output is $1$ corresponds to a set cover.
The player then derives a prize of $\hat{m}$
from contests in $M_2$. If her output is $1$ along $\kappa'>\kappa$ activities, she incurs a cost 
of $\kappa'\cdot (\hat{m}+1)$ and receives prizes
of total value $\kappa'\cdot (\hat{m}+1/2)$ from
contests in $M_1$, so her total payoff 
is $\hat{m}-\kappa'/2< \hat{m}-\kappa/2$, a contradiction. Thus, the player's output is 
$1$ along at most $\kappa$ activities, and 
these activities correspond to a set cover.

\textbf{Budget.} The construction for the budget model is the same as the cost model, except that the player does not have any cost for producing output along any activity but has a total output budget of $\kappa$.

As argued before, the contests in $M_1$ are much more valuable than the ones in $M_2$, and contests in $M_1$ award prizes only if a player produces an output of $1$ along individual activities; therefore, the player selects $\kappa$ activities and produces an output of $1$ along these. Now, the player would also like to select these $\kappa$ activities so as to win as many of the contests in $M_2$, and if possible, all. This is equivalent to deciding if the input instance of {\sc Set Cover} is a yes-instance.
\end{proof}
We note that in a single-player case finding a best response is equivalent to finding a PNE. We obtain the following corollary.

\begin{corollary}
In the linear multi-activity model, 
the problem of computing a PNE is {\em NP}-hard. 
This holds both for the cost model and for the budget model.
\end{corollary}

Theorem~\ref{thm:hardBestResp} proves that it is hard to compute an exact best response. The next question to consider is whether 
a player is able to efficiently compute an approximate solution that is arbitrarily close to the optimal, i.e., whether our problem admits a polynomial-time approximation scheme. In the next theorem, we rule out such a possibility for the budget model; we discuss the cost model subsequently.

\begin{theorem}\label{thm:hardApproxBestResp}
In the linear multi-activity budget model, there is no polynomial-time approximation scheme for best-response, unless {\em P = NP}.
\end{theorem}
\begin{proof}
We prove this result by providing a reduction from \textsc{MAX-2-SAT-3}. In an instance of the \textsc{MAX-2-SAT-3} problem, we are given a 2-CNF formula where each variable occurs at most $3$ times, and the objective is to find an assignment of the variables to satisfy as many clauses of the 2-CNF formula as possible. It is known that it is NP-hard to approximate this problem beyond a constant factor~\cite{berman1999some}. 

Consider an instance of \textsc{MAX-2-SAT-3} with $\hat{n}$ variables $x_1, x_2, \ldots, x_{\hat{n}}$. Let there be $\hat{m}$ clauses in the 2-CNF formula; w.l.o.g. assume that $\hat{m} \ge \hat{n}$. We construct an instance of the multi-activity budget game with one player, $k = 2 \hat{n}$ activities, and $m = \hat{m} + 4 \hat{n}$ contests. The player has a budget of $\hat{n}$ that she can allocate across any of the $2\hat{n}$ activities. Each contest awards a prize of $1$.
\begin{itemize}
    \item Activities: Corresponding to each variable in the 2-CNF formula, we have two activities in the game. For variable $x_i$, we have activity $i$ with output $b_i$, corresponding to the literal $x_i$, and we have activity $\hat{n}+i$ with output $b_{\hat{n}+i}$, corresponding to the literal $\neg x_i$. We sometimes denote $b_{\hat{n}+i}$ by $b_i'$ for a cleaner presentation.
    \item Contests: The $m = \hat{m} + 4 \hat{n}$ contests are of two types:
    \begin{enumerate}
        \item Contests $M_1$. There are $\hat{m}$ contests of this type, and these contests correspond to the clauses in the 2-CNF formula. For a clause $x_i \land x_j$, we have a contest with condition $b_i + b_j \ge 1$. Similarly, for a clause $x_i \land \neg x_j$, there is a contest with condition $b_i + b_j' \ge 1$, and so on for the other types of clauses. A contest in $M_1$ can be identified by the associated pair of activities $(i,j) \in [2 \hat{n}] \times [2 \hat{n}]$.
        \item Contests $M_2$. There are $4\hat{n}$ contests of this type, and they correspond to the $2\hat{n}$ possible literals in the 2-CNF formula. For each $i \in [\hat{n}]$, there are two contests with condition $b_i \ge 0$ and two with condition $b_i' \ge 0$.
        % \item Contests $M_3$. There are $\hat{n}$ contests of this type, and they correspond to the $\hat{n}$ variables in the 2-CNF formula. For each $i \in [\hat{n}]$, there is a contest with criteria $b_i + b_i' \ge 0$.
    \end{enumerate}
\end{itemize}
As each contest has a prize of $1$, the objective of the player is to satisfy as many contests as possible.

Let us assume that for linear multi-activity budget games, we have a polynomial-time algorithm that approximates the best response by a factor $\gamma \in (0,1]$.
Let $\bb$ be a solution for the instance of the problem we just constructed, found in polynomial time using this approximation algorithm.

From this approximate solution $\bb$, we construct a $\{0,1\}$-integral approximate solution with at least as good an approximation ratio as $\bb$, as described below:
\begin{enumerate}
    \item If there is an $i \in [2 \hat{n}]$ such that $b_i > 1$, set $b_i = 1$. Notice that this transformation does not affect the number of satisfied contests. In the subsequent transformations of $\bb$, we will not touch these $b_i$ values (where $b_i = 1$) and the contests that contain them. So, the contests where they show up will remain satisfied. Let these contests be denoted by $M^{(1)}$.
    \item Let $M_1^{(2)}$ denote the contests in $M_1 \setminus M^{(1)}$ that are satisfied by $b$. Do the following updates to $\bb$ and $M_1^{(2)}$ until  $M_1^{(2)} = \emptyset$:
    \begin{itemize}
        \item Take an arbitrary contest $(i,j)$ in $M_1^{(2)}$. We know that the following conditions hold: $b_i + b_j \ge 1$, $b_i < 1$, and $b_j < 1$. 
        \item Set $b_i = 1$ and $b_j = 0$. As the value of $b_i$ increases, the contests that contain $b_i$ and were satisfied before this update remain satisfied after this update. On the other hand, as every variable may occur in at most three clauses, $b_j$ may occur in at most two more contests in $M_1^{(2)}$ in addition to the current contest $(i,j)$. These contests become unsatisfied as a result of this transformation, but they are compensated by the two contests in $M_2$ that correspond to $b_i$, which were unsatisfied before this update, but become satisfied after this update.
        \item Remove all contests from $M_1^{(2)}$ that correspond to the activities $i$ or $j$, i.e., set $M_1^{(2)} = M_1^{(2)} \setminus \{ (\ell, t) \mid  \{\ell, t\} \cap \{i,j\} \neq \emptyset \}$.
    \end{itemize}
    As the size of $M_1^{(2)}$ decreases after each update without decreasing the total number of satisfied contests, the process terminates with a solution as good as before.
    \item As a result of the previous step, there is no contest in $M_1$ that is satisfied but has an output strictly less than $1$ for both of its activities. In other words, for any contest $(i,j) \in M_1$, $b_i + b_j \ge 1 \implies \max(b_i, b_j) = 1$. Moreover, none of the contests in $M_2$ can be satisfied by an activity $i$ with $b_i < 1$. So, we can safely set $b_i = 0$ for all $i$ with $b_i < 1$, without decreasing the number of satisfied contests.
\end{enumerate}
Thus, we can assume without loss of generality that the solution for the instance of the linear multi-activity budget game is $\{0,1\}$-integral. We can also assume that $\sum_{i \in 2 \hat{n}} b_i = \hat{n}$, because setting additional $b_i$ values to $1$ does not decrease the objective. 

As mentioned before, \textsc{MAX-2-SAT-3} is NP-hard to approximate beyond a constant factor, even when the number of clauses is of the same order as the number of variables, i.e., $\hat{m} = \Theta(\hat{n})$, as proved by \citet{berman1999some}, given in the theorem below. 

\begin{theorem}\cite{berman1999some}\label{thm:bk}
For any $0 < \epsilon < 1/2$, it is {\em NP}-hard to decide whether an instance of {\sc MAX-2-SAT-3} with $\hat{m} = \mu_1 \hat{n}$ clauses has a truth assignment that satisfies $ (\mu_2 + 1 - \epsilon) \hat{n}$ clauses, or every truth assignment satisfies at most $(\mu_2 + \epsilon) \hat{n}$ clauses, where $\mu_1$ and $\mu_2$ are two positive constants.\footnote{$\mu_1 = 2016$ and $\mu_2 = 2011$. \citet{berman1999some} call the problem \textsc{3-OCC-MAX-2SAT} instead of \textsc{MAX-2-SAT-3}.}
\end{theorem}
Theorem~\ref{thm:bk} proves that \textsc{MAX-2-SAT-3} cannot be approximated better than a factor $(\mu_2 + 1)/\mu_2 - \epsilon$. Now, if an instance of the $\textsc{MAX-2-SAT-3}$ problem has a truth assignment that satisfies $\gamma \hat{n}$ clauses, then the constructed instance of the linear budget game has a best response that satisfies $(\gamma + 4) \hat{n}$ contests. So, for any $0 < \epsilon < 1/2$, it is NP-hard to decide whether an instance of the linear budget game with $m = \hat{m} + 4 \hat{n} = (\mu_1 + 4)\hat{n}$ contests has a best response that satisfies $ (\mu_2 + 5 - \epsilon) \hat{n}$ contests, or it can be at most $(\mu_2 + 4 + \epsilon) \hat{n}$. This gives us an approximation ratio of $(\mu_2 + 5)/(\mu_2 + 4) - \epsilon$.

% Let this constant factor be $\hat{\gamma} \in (0,1)$. Additionally, this result holds even when it is given that the optimal solution is a constant factor of the number of variables in the CNF formula. Formally, it is hard to tell whether an optimal solution is $\le \hat{\gamma}  \mu  \hat{n}$ or $\ge \mu  \hat{n}$, for some constant $\mu \in (0,1)$.

% Using this result, we get the approximation ratio of the linear multi-activity budget game to be $\gamma \le \frac{\hat{\gamma} \mu + 2}{\mu + 2}$, which is a constant. Because, if the instance of the $\textsc{MAX-2-SAT-3}$ problem has the optimal objective value $\mu \hat{n}$, then the constructed instance of the linear budget game has the optimal objective value $(\mu + 2) \hat{n}$. If $\gamma > \frac{\hat{\gamma} \mu + 2}{\mu + 2}$, then the approximate solution for the game will have an objective value $\frac{\hat{\gamma} \mu + 2}{\mu + 2}  (\mu + 2) \hat{n} = \hat{\gamma} \mu \hat{n} + 2 \hat{n}$. So, strictly more than $\hat{\gamma} \mu \hat{n}$ contests from $M_1$ need to be satisfied, which provides a solution for the instance of the $\textsc{MAX-2-SAT-3}$ problem strictly better than $\hat{\gamma}$ times the optimal, contradiction.
\end{proof}

Theorem~\ref{thm:hardApproxBestResp} proves that the problem of finding a best response in the linear multi-activity budget model does not admit a polynomial-time approximation scheme. For restricted versions of the model, a constant factor approximation can be found. For example, if the contests have $\{0,1\}$ weights for the activities, and the player has a budget that she can distribute across any of the activities (the instance constructed in Theorem~\ref{thm:hardApproxBestResp} satisfies these conditions), then the problem becomes a submodular maximization problem with a polynomial-time constant-factor approximation algorithm. However, we feel that a 
constant-factor approximation result is of limited usefulness in the context of
computing a best response or a Nash equilibrium.

For the multi-activity cost model, the problem of approximating a best response is less well-behaved, because a player's utility may become negative. If a player produces a $0$ output for all the activities, she has a utility of $0$. We can create instances where it is NP-hard to decide if there exists an action that gives strictly positive utility to the player, which shows that this problem is inapproximable. The proof proceeds by modifying the construction in the proof of Theorem~\ref{thm:hardBestResp}: we tweak the costs to make sure that the utility of the player is strictly positive if and only if she finds a set cover of size $\kappa$ (or smaller), which is NP-hard.

% As proved in the theorem above, best-response is NP-hard in multi-activity games. It is easy to observe that best response is easy in single-activity games: the player selects an activity among the $k$ activities, and then for the selected activity, the player selects the level of output (for which they essentially have to select among at most $m$ output levels, depending upon the minimum criteria to win the contests).

==> ec/conclusion.tex <==
\section{Future Work}
%In this paper, we studied a practically relevant model of contests and analyzed its properties: existence of equilibria, price of anarchy, and the computational complexity of finding an equilibria.

An important future direction is to find computationally tractable, yet relevant in real-life, special cases of the model. For the multi-activity model, the problem is NP-hard even with a constant number of players, as shown in Section~\ref{sec:multiActivity}. However, in the single-activity model, the problem becomes tractable with a constant number of players: the number of actions for a player is polynomial in the number of activities and contests, so we can explicitly construct a polynomial-size normal-form game and find the PNE; this puts our problem in XP. A thorough investigation of fixed-parameter tractability w.r.t. relevant parameters, including the number of contests, activities, and players, and their combinations, is a promising research direction. One can also study the complexity of an approximate equilibrium for the models; some PLS-complete problems have polynomial-time algorithms for an approximate PNE, while for others, finding an approximate PNE is also PLS-complete~\cite{chien2011convergence,skopalik2008inapproximability}.

Another direction is to apply the three-level model, player--activity--contest, to contests with other types of prize allocation rules rather than the equal-sharing allocation, such as rank-based allocation, proportional allocation, etc. For these contests one may study properties of the equilibria and the computation complexity. We also believe that there is much to explore regarding the computational complexity of simultaneous contests, in general.





% \abheek{reduction from an arbitrary congestion games? gap introducing reduction from FLIP?}

% \paul{As we discussed, it may be of interest to find a generalisation to which we can reduce the problem of finding a mixed NE of an explicit congestion game.}

% \paul{Another item: I don't think there's any issue of social welfare, right now, in these games, is that right? The $n$ players spend their budgets of 1 without any cost, and all prizes are awarded. But in a mixed equilibrium, there may be contests that with positive probability, no-one enters.}
% \abheek{Answer to Paul's second question, added a portion about social welfare, Section~\ref{sec:pnepoa}.}

==> ec/intro.tex <==
\section{Introduction}
Contests are games where players, who are assumed to be strategic, make costly and irreversible investments to win valuable prizes~\citep{vojnovic2015contest}. Typically, the prizes have monetary value, which incentivizes the players to make the costly investments. In some scenarios, the prizes may be associated with reputation and social status. For example, many online forums and websites depend upon user-generated content to provide value to their customers, and award badges, which do not have any monetary value but provide social reputation (e.g., StackOverflow and Quora);
see, e.g., \cite{immorlica2015social}.

In the presence of multiple simultaneous contests, 
each player may explicitly select one or more contests and invest efforts so as to win
the associated prizes. However, sometimes contest participation is implicit:
players engage in various activities, and each contest awards prizes to some of the players based on their performance in a specific subset of activities.  

Consider, for instance, the setting where several social media platforms or news websites compete to attract customers. The potential customers are not homogeneous:
e.g., some may be interested in politics, while others focus on sports or technology.
It is therefore natural to model this setting as a set of simultaneous contests, 
with each individual contest corresponding to a group of customers with similar preferences. The platforms can take actions that make them more attractive to potential customers. Indeed, some of the actions, such as improving the interface, or increasing the update frequency, may impact the platform's performance with respect to several customer groups. That is, we can think of platforms as engaging in several {\em activities}, with their performance in each contest depending on the effort they invest in these activities. Different customer groups may value different mixtures of activities in different ways: e.g., while consumers of financial and sports news care about frequent updates, those who read the gossip column are happy with daily or even weekly updates. Thus, by increasing her investment in an activity, a player may 
improve her performance in several---but not all---contests.

In this work, we put forward a formal model that can capture scenarios of this type. In our model, there are several players and several simultaneous contests, as well as a set of activities. Each player selects their effort level for each activity (and may incur a cost for doing so, or face budget constraints), and each contest $j$ has its own success function, which specifies combinations of effort for each activity that are sufficient to succeed in $j$. In addition to that, we assume that each contest allocates identical prizes to all agents
that meet its criteria\footnote{The motivation for equal sharing allocation is somewhat similar to that of proportional allocation (e.g., in \citet{tullock1980efficient} contests), except that equal sharing becomes relevant in situations where the contests try to use rules (or criteria) to decide allocation.}: 
e.g., if, to win contest $j$, it suffices to produce $2$ units along activity $\ell$, then the player who produces $3$ units along $\ell$ and the player who produces $30$ units along $\ell$ receive the same prize from $j$; however,  the value of the prize in contest $j$ may depend of the number of players who 
meet the criteria of $j$. We refer to this setting as {\em multi-activity games}. 

From the perspective of the player, we distinguish between two models: (1) the \textit{cost model}, which has cost functions for producing output, and (2) the \textit{budget model}, which has generalized budget constraints (feasible subsets of the space). The cost functions and the budget constraints may be different across players, capturing the fact that some players may be able to perform better in some activities compared to others.

Our model is very general: we impose very mild and natural constraints on the contests' success functions and prize allocation rules. In particular, we assume that the total value of the prizes allocated to the winners of each contest is a monotonically non-decreasing and concave function of the number of winners;
these assumptions capture the idea that the value of an award decreases as it gets awarded to a larger number of players (see, e.g., \cite{immorlica2015social}).
A specific instantiation of this model is a contest that has a \textit{fixed total prize} of $V$, and every winner gets a share of $V/k$ if there are $k$ winners. 


Besides our social media platform example, there are several other situations that can be modeled using contests with equal sharing allocation of prizes, where players compete by engaging in activities valued by multiple contests. For instance,  funding agencies are generally not able to \textit{perfectly discriminate} among the applicants to select the most deserving one. They might score candidates based on attributes such as strength of proposal, publication history, and management experience, and allocate their budget to one of the eligible candidates or distribute it among them. Because of this uniform distribution of prize, from the perspective of an expected utility maximizing applicant, this situation can be approximated using a contest with an equal sharing allocation with a fixed total prize. 


\subsection{Our Results}
We observe that, under mild assumptions, multi-activity games are \textit{exact potential games}~\cite{monderer1996potential} (see Definition~\ref{def:potentialGames}). This guarantees the existence of a pure-strategy Nash equilibrium (PNE). 
Moreover, an approximate PNE can be computed in pseudo-polynomial time. In fact, a sequence of $\epsilon$-better/best\footnote{An $\epsilon$-better response move increases the utility of a player by at least $\epsilon$.} response moves converges to an $\epsilon$-PNE, with number of steps proportional to $1/\epsilon$ (and pseudo-polynomial in other parameters).
For the budget model, for the natural definition of social welfare in these games, we observe that the price of anarchy (PoA)\footnote{The price of anarchy is the ratio between the social welfare of the optimal solution and the social welfare of an equilibrium solution, in worst case over instances of the problem and corresponding equilibrium solutions.} is at most $2$, and this bound is tight. 
However, for the cost model, for meaningful definitions of social welfare, the price of anarchy can be infinite. 

% For the budget model, for the natural definition of social welfare in these games, we observe that the social welfare is a submodular function (as defined by \citet{vetta2002nash}). And, using \citet{vetta2002nash}'s result, the budget model has a price of anarchy (PoA) at most $2$ (tight). 
%
%Only the PoA results differ between the cost and the budget models, as mentioned in the previous paragraph.
% This result on PoA is the only result that is different between the cost and the budget models. Therefore, for the rest of this section, we focus only on the budget model. 

%On the other hand, all our negative results are proved for the case of an equal sharing allocation with a fixed total prize (where every winner gets a $1/k$ fraction of the prize if there are $k$ winners). 
% Therefore, for a clearer presentation, we do not explicitly mention fixed total prize every time we mention the (negative) results.

We then focus on a specific instantiation of this model, where the contests' criteria and the players' budget constraints are all linear; let us call this model the \textit{linear model}. (Here, we discuss the results for the budget model. With similar assumptions, similar results hold for the cost model as well.)
%A simple linear budget constraint bounds the total output of a player across the activities. The criterion of a contest says that a (contest-specific) weighted combination of the outputs should be above some threshold (say $1$, w.l.o.g.). We prove all our complexity lower results for this restricted model.
%Our positive results hold for general equal sharing allocation, where the value of a contest's prize to an individual player (weakly) decreases as the number of winners increases. 
We show that, for the linear model, it is NP-hard for a player to best respond to the strategies of other players. This hardness result holds even for a game with only one player; in other words, the hardness is due to the optimization problem that a player faces while playing the game. We also prove that there exists no polynomial-time approximation scheme unless P$=$NP. (Here, NP-hardness for best-response directly implies NP-hardness for equilibrium computation.)

The NP-hardness result for best-response motivates us to further restrict our model: 
we assume that a player can produce output only along a small (polynomial) number of portfolios of activities. Mathematically, a portfolio corresponds to a direction in the activity space along which a player can produce output. This restricted model captures salient features of the original model: e.g., it maintains the property that the contests can have overlapping criteria.

With a simple transformation of the activity space, the portfolio model can be converted to an equivalent model where a player produces output only along one activity, i.e., only along the axes, where an activity in the new model corresponds to a portfolio in the old model. In our discussion, we call this new model the \textit{single-activity model} to differentiate it from the original model, which we call the \textit{multi-activity model}.

The positive results of the multi-activity model automatically carry over to the single-activity model. Additionally, it is computationally easy for the players to best respond in the single-activity model. However, we get a different hardness result. Even for a linear model, it is PLS-complete to compute a PNE and (PPAD$\cap$PLS)-complete to compute a mixed-strategy Nash equilibrium (MNE). 
This hardness result adds another natural and practically relevant problem to the class of (PPAD$\cap$PLS)-complete problems, which includes finding a fixed-point of gradient descent~\cite{fearnley2021complexity} and finding an MNE of explicit congestion games~\cite{babichenko2021settling}. Indeed, the class of single-activity games is a strict subset of the class of explicit congestion games: a contest awards a $1/k$ fraction of a fixed prize to each winner if there are $k$ winners, but a congestion game can have a cost that is an arbitrary function of the number of winners.

The rest of this paper is organized as follows. 
After summarizing the related work (Section~\ref{sec:related}), in Section~\ref{sec:modelpnepoa} we introduce the general multi-activity model. We also prove the existence of PNE, the pseudo-polynomial convergence of $\epsilon$-best-response dynamics to $\epsilon$-PNE, and present our PoA results. In Section~\ref{sec:multiActivity} we establish the hardness of best-response in linear multi-activity models. Section~\ref{sec:singleActivity} focuses on the single-activity model and presents our results on PLS-completeness and (PPAD$\cap$PLS)-completeness. 

% All omitted proofs are provided in the appendix.

\subsection{Related Work}\label{sec:related}
The linear budget model with a fixed total prize has previously been studied by \citet{may2014filter}, to model situations such as the social media platform example discussed earlier. Their theoretical results are similar to our positive results: 
(i) they prove existence of PNE by showing that the game is an exact potential game; (ii) they establish a PoA bound of $2$. For (i), existence of PNE, we give a much simpler proof by explicitly constructing the potential function that lifts these results to our general model. The proof also makes it transparent that the PNE exists because of the equal sharing property of the contests (the \textit{congestion} property), and the other restrictions of the model of \citet{may2014filter}---the linear budgets constraints, the linear criteria of contests, and the fixed total prize---are not necessary for the result. Moreover, the proof clarifies that using the budget model is also non-essential, as the result holds for the cost model as well. For (ii), the PoA bound, \citet{may2014filter} prove the result from first principles. In contrast, we use the result of \citet{vetta2002nash} for submodular social welfare functions to derive the same result in our---much more general---setting.
\citet{may2014filter} do an empirical study and show that the real-life behavior of social media curators resembles the predictions of the model. 
  \citet{bilo2019project} consider a model similar to the single-activity model of our paper and show an inclusion in the class PLS (but no hardness results).
%  They introduced a budget version of the model to study competition among social media curators to acquire followers. They prove the existence of a PNE by showing equivalence to an exact potential game (see Definition~\ref{def:potentialGames}), and give the PoA bound of $2$. They also do an empirical study and show that the real-life behavior resembles the predictions of the model. The book by \citet{vojnovic2015contest}, Chapter 5 Section 5.5, presents a slightly generalized model with similar results; our budget model generalizes both these budget models. To our knowledge, the work of \citet{may2014filter} is the only paper that studies a three-component player--activity--contest model.

% \abheek{\citet{vetta2002nash} is not necessary to discuss here. It is a technical result we use in our proof.}

Models of simultaneous contests that do not have activities (i.e., the players directly produce outputs for individual contests, or, equivalently, there is a one-to-one mapping between the activities and the contests) have been extensively studied. Cost-based models where the prizes are awarded based on the ranks of players have been considered by \cite{amann2008parallel,archak2009optimal,bapna2010vertically,dipalantino2009crowdsourcing}, including empirical work by \cite{archak2009optimal,dipalantino2009crowdsourcing,lakhani2010topcoder,yang2008crowdsourcing}. Colonel Blotto games, where the players have budget constraints and the prize is awarded to the highest-output player for each contest, were introduced by \citet{borel1921analyse}, and have received a significant amount of attention in the literature (e.g., \cite{borel1938application,tukey1949problem,gross1950continuous,blackett1954some,blackett1958pure,bellman1969colonel,shubik1981systems,roberson2006colonel,hart2008discrete,adamo2009blotto,roberson2006colonel,hortala2012pure,washburn2013or}). Simultaneous contests with proportional allocation have been studied by, e.g., \cite{feldman2005price,zhang2005efficiency,palvolgyi2010strategic}.

The complexity class PLS (Polynomial Local Search) and the concepts of PLS-hardness and PLS-completeness were introduced by \citet{johnson1988easy}. PLS consists of discrete local optimization problems whose solutions are easy to verify (the cost of a given solution can be computed in polynomial time and its local neighborhood can be searched in polynomial time). Similarly to NP-hard problems, PLS-hard problems are believed to be not solvable in polynomial time. Several natural problems, such as finding a locally optimal solution of {\sc Max-Cut}, were shown to be PLS-complete by \citet{schaffer1991simple}. The problem of finding a PNE in explicit congestion games (which always have PNE) is also PLS-complete~\cite{fabrikant2004complexity}, from which it follows that better or best response dynamics take an exponential time to converge in the worst case.

The class PPAD (Polynomial Parity Arguments on Directed graph) was introduced by \citet{papadimitriou1994complexity}. Like PLS problems, PPAD problems always have solutions. For PPAD, the existence of a solution is based on a parity argument: In a directed graph where each vertex has at most one predecessor and one successor, 
if there exists a source vertex (i.e., a vertex with no predecessor), then
there exists some other degree-1 vertex.
One of the most well-known results in algorithmic game theory
is that the problem of finding a mixed-strategy Nash equilibrium (MNE) is PPAD-complete~\cite{daskalakis2009complexity,chen2009settling}. 

Recent work has determined the complexity of computing an MNE of an explicit congestion game. The class PPAD$\cap$PLS represents problems that can be solved both by an algorithm that solves PPAD problems and by an algorithm that solves PLS problems. 
Finding an MNE of an explicit congestion game is in PPAD$\cap$PLS: indeed,  this problem can be solved either by finding a PNE (which is also an MNE) using an algorithm for PLS problems or by computing an MNE using an algorithm for PPAD problems.
Recently, \citet{fearnley2021complexity} proved that finding a fixed-point of a smooth $2$-dimensional function $f : [0,1]^2 \rightarrow \bR$ using gradient descent is complete for the class PPAD$\cap$PLS; based on this result, \citet{babichenko2021settling} proved that finding an MNE of an explicit congestion game is also (PPAD$\cap$PLS)-complete.
PLS-complete, PPAD-complete, and (PPAD$\cap$PLS)-complete problems are considered to be hard problems with no known polynomial-time algorithms.

==> ec/model-pne-poa.tex <==
\section{General Model, Pure Nash Equilibrium, and Price of Anarchy}\label{sec:modelpnepoa}
In this section, we formally define the general multi-activity model, prove the existence of pure Nash equilibria, and show that the price of anarchy (PoA) is $2$ for the budget variant of the model and $+\infty$ for the cost variant.

We consider a set of $n$ players, $N = [n]$, who simultaneously produce output along $k$ activities, $K = [k]$. There are $m$ contests, $M = [m]$, which award prizes to the players based on their outputs. The contests may have different prizes and may value the activities differently.
%Typically, a player's output along some activity may make various contributions to their ability to win different contests.

We study two models: in one, the players have output production costs; and in the other, the players have generalized output budgets. Player $i \in N$ chooses an output vector $\bb_i = (b_{i,\ell})_{\ell \in K} \in \bR_{\ge 0}^k$.
\begin{itemize}
    \item \textbf{Cost.} Player $i$ incurs a cost of $c_i(\bb_i)$ for producing $\bb_i$, where $c_i : \bR_{\ge 0}^k \rightarrow \bR_{\ge 0}$ is a non-decreasing cost function with $c_i(\bm{0}) = 0$ (normalized). 
    % We shall prove our computational hardness and unbounded PoA results for a simpler model with linear cost functions, where $c_i(\bb_i) = \sum_{\ell \in K} c_{i,\ell} b_{i,\ell}$, but the existence of PNE shall hold for the general model.
    \item \textbf{Budget.} The player does not incur any cost for the output vector $\bb_i$, but $\bb_i$ is restricted to be in a set $\cB_i \subseteq \bR_{\ge 0}^k$. We assume that $\bm{0} \in \cB_i$, i.e., players are always allowed to not participate. 
    % In this model too, the positive results hold for general $\cB_i$, but the negative results hold for a simple model where the players are identical and with a fixed budget that can be split amongst the activities. 
\end{itemize}
Let $\bb = (\bb_i)_{i \in N} = (b_{i,\ell})_{i \in N, \ell \in K}$. 
Each contest $j\in M$ is associated with a pair of functions 
$f_j: \bR_{\ge 0}^k \rightarrow \bR_{\ge 0}$ 
and
$v_j: \bN \rightarrow \bR_{\ge 0}$.
The function $f_j$, which is an increasing function such that $f_j(\bm{0}) = 0$, determines the set of winners of contest $j$: we say that player $i$ {\em wins} contest $j$ if $f_j(\bb_i) \ge 1$ and set
\[ 
    N_j(\bb) = \{ i\in N \mid f_j(\bb_i) \ge 1 \}.
\]
 Let $n_j(\bb) = |N_j(\bb)|$. 
 The function $v_j$ determines how the prizes are allocated: each player 
 in $N_j(\bb)$ receives a prize of $v_j(n_j(\bb))$. 
 The total prize allocated by contest $j$ is then $n_j(\bb)\cdot v_j(n_j(\bb))$; 
 we assume that this is a weakly concave non-decreasing function of the number of winners. Formally, we require that $x \cdot v_j(x)$ is 
 (i) non-decreasing, i.e., $\frac{d (x \cdot v_j(x))}{dx} \ge 0$, and (ii) weakly concave, i.e., $\frac{d^2 (x \cdot v_j(x))}{dx^2} \le 0$. Both of these assumptions are important for our price of anarchy bounds. Some examples of functions $v_j$ that satisfy these conditions are:
\begin{itemize}
    \item $x \cdot v_j(x) = x$ or $v_j(x) = 1$. Here, the total value of the prize scales linearly with the number of winners, i.e., the prize awarded to a winner does not change as the number of winners increases.
    \item $x \cdot v_j(x) = 1$ or $v_j(x) = 1/x$. Here, the total value of the prize remains constant, i.e., the prize awarded to a winner decreases and is equal to the inverse of the number of winners.
    \item $x \cdot v_j(x) = \sqrt{x}$ or $v_j(x) = 1/\sqrt{x}$. This sits between the previous two examples. Here, the total value of the prize increases, but the prize awarded to a winner decreases as the number of winners increases.
\end{itemize}
% Again, we shall prove the negative results for a simpler model where $v_j(\ell) = V_j/\ell$ for some constant $V_j > 0$ (fixed total prize) and where $f_j$ is a linear function given as $f_j(\bb_i) = \sum_{\ell \in K} w_{j,\ell} b_{i,\ell}$ where $w_{j,\ell} \in \bR_{\ge 0}$. But, the positive results hold for the general case.

The utility of a player $i$ in the cost model and the budget model is, respectively,
\begin{equation*}
    u_i(\bb) = \sum_{j \in M} v_j(n_j(\bb)) \cdot \b1\{i \in N_j(\bb)\} - c_i(\bb_i)\qquad\text{and}\qquad u_i(\bb) = \sum_{j \in M} v_j(n_j(\bb))\cdot \b1\{i \in N_j(\bb)\},
\end{equation*}
where $\b1\{\ldots\}$ is the indicator function.

We will be interested in stable outcomes of multi-activity games, 
as captured by their Nash equilibria.

\begin{definition}[Pure-Strategy Nash Equilibrium (PNE)]
A pure strategy profile $\bb = (\bb_i, \bb_{-i})$ is a {\em pure Nash equilibrium (PNE)} if for every $i \in N$ and every action $\bb_i'$ of player $i$ we have $u_i(\bb_i', \bb_{-i}) \le u_i(\bb)$.
\end{definition}

% \begin{definition}[Price of Anarchy (PoA)]\label{def:poa}
% Given a social welfare function, $sw$, the price of anarchy is the ratio between the social welfare of the optimal solution and the social welfare of an equilibrium solution, in worst case over possible instance of the problem and possible equilibria. Formally, $PoA = $ 
% \end{definition}


\subsection{Existence of Pure-Strategy Nash Equilibrium}
We start by showing that multi-activity games are exact potential games.
We then use the classic result of 
\citet{monderer1996potential} to conclude that multi-activity games
always have pure Nash equilibria. 
%which corresponds to the pure strategy profile that maximizes a potential function.
\begin{definition}[Exact Potential Games]\label{def:potentialGames}\cite{monderer1996potential}
A normal form game is an {\em exact potential game} if there exists a potential function $\phi$ such that for any player $i$ with utility function $u_i$,
any two strategies $\bb_i$ and $\bb_i'$ of player $i$, and any strategy profile $\bb_{-i}$ of the other players it holds that
\[ u_i(\bb_i', \bb_{-i}) - u_i(\bb_i, \bb_{-i}) = \phi(\bb_i', \bb_{-i}) - \phi(\bb_i, \bb_{-i}). \]
\end{definition}
\begin{theorem}\cite{monderer1996potential}
Exact potential games always have a pure-strategy Nash equilibrium.
Indeed, every pure strategy profile that maximizes $\phi$ 
is a PNE.
\end{theorem}

We define the potential functions for the multi-activity budget and cost games as, respectively,
\begin{equation}\label{eq:potFun}
    \phi_B(\bb) = \sum_{j \in M} \sum_{\ell \in [n_j(\bb)]} v_j(\ell) \qquad
    \text{and}\qquad 
    \phi_C(\bb) = \sum_{j \in M} \sum_{\ell \in [n_j(\bb)]} v_j(\ell) - \sum_{i \in N} c_i(\bb_i);
\end{equation}
we omit the subscripts $B$ and $C$ if they are clear from the context. We shall now use these potential functions to prove the existence of PNE in multi-activity games. In Section~\ref{sec:singleActivity}, we shall also use these to study the complexity of computing equilibria in these games. 
\begin{theorem}\label{thm:multPNE}
A multi-activity budget/cost game is an exact potential game, and hence, has a pure-strategy Nash equilibrium.
\end{theorem}
\begin{proof}
We shall prove the result for the cost game. The budget game can be reduced to the cost game by endowing it with cost function $c(\cdot)$ that is always equal to $0$ (the presence of the budget constraint does not affect the proof).

Let player $i$ make a move by changing its strategy from $\bb_i$ to $\bb_i'$, and let $\bb_{-i}$ be the pure strategy profile of the other players. Let $S \subseteq M$ and $S' \subseteq M$ be the contests that player $i$ wins for strategy profiles $\bb = (\bb_i, \bb_{-i})$ and $(\bb_i', \bb_{-i})$, respectively. 
We have 
$$
n_j(\bb_i', \bb_{-i}) = 
\begin{cases}
n_j(\bb) - 1 \quad\text{ if $j \in S \setminus S'$}\\
n_j(\bb) + 1 \quad\text{ if $j \in S' \setminus S$}\\
n_j(\bb) \quad\text{ in all other cases}.
\end{cases}
$$
The change in the potential $\phi(\bb_i', \bb_{-i}) - \phi(\bb)$ can be expressed as
\begin{align*}
    &\  \sum_{j \in M} \left( \sum_{\ell \in [n_j(\bb_i', \bb_{-i})]} v_j(\ell) - \sum_{\ell \in [n_j(\bb)]} v_j(\ell) \right) - \left(  c_{i}(\bb_i') - c_i(\bb_i)  \right) + \sum_{q \in N \setminus \{i\}}  \underbrace{\left(  c_{q}(\bb_{q}) -  c_{q}(\bb_{q}) \right)}_{= 0}, \\
    &= \underbrace{\left(\sum_{j \in S' \setminus S} v_j(n_j(\bb_i', \bb_{-i})) -  c_i(\bb'_i)\right)}_{u_i(\bb_i', \bb_{-i})}  - \underbrace{\left( \sum_{j \in S \setminus S'}v_j(n_j(\bb)) - c_i(\bb_i) \right)}_{u_i(\bb)}\ ,
\end{align*}
which is exactly equal to the change in the utility of the player $i$.
\end{proof}
Note that the proof of Theorem~\ref{thm:multPNE} only depends upon the equal sharing property of the contests (and the fact that a player's cost
only depends on her own action).

\subsection{Approximate Pure-Strategy Nash Equilibrium using Better-Response}
The characterization in Theorem~\ref{thm:multPNE} 
is very useful for finding approximate equilibria 
of multi-activity games. 
%are exact potential games, we can easily observe that an $\epsilon$-PNE can be found using $\epsilon$-better-response moves. In an $\epsilon$-PNE, no player can benefit by more than $\epsilon$ (additive) by deviating. And, we shall call a better-response move $\epsilon$-better-response it increases the utility of a player by more than $\epsilon$.
\begin{definition}[$\epsilon$-Pure-Strategy Nash Equilibrium]
A pure strategy profile $\bb = (\bb_i, \bb_{-i})$ is an {\em $\epsilon$-PNE} if for every $i \in N$ and every action $\bb_i'$ of player $i$ we have $u_i(\bb_i', \bb_{-i}) \le u_i(\bb) - \epsilon$.
\end{definition}
\begin{definition}[$\epsilon$-Better-Response]
For a pure strategy profile $\bb = (\bb_i, \bb_{-i})$, a player $i \in N$, and an action $\bb_i'$ of player $i$, the move from $\bb_i$ to $\bb_i'$ is an {\em $\epsilon$-better-response move} if $u_i(\bb_i', \bb_{-i}) > u_i(\bb) + \epsilon$.
\end{definition}
From the definitions above, it is immediate that a pure strategy profile is an $\epsilon$-PNE  if and only if it does not admit any $\epsilon$-better-response moves.  Now, as multi-activity games are exact potential games,
each $\epsilon$-better-response increases the potential 
by at least $\epsilon$. As the potential function is bounded from above, a sequence of $\epsilon$-better-response moves necessarily terminates, 
and the resulting profile is an $\epsilon$-PNE.
\begin{corollary}\label{thm:pseudoPolyBR}
In multi-activity games, any sequence of $\epsilon$-better-response moves arrives to an $\epsilon$-PNE in at most $n \cdot m \cdot (\max_{j} v_j(1)) / \epsilon$ steps.
\end{corollary}
\begin{proof}
%Both for the cost model and for the budget model, 
The potential function is bounded from above by $\phi(\bb) \le \sum_{j \in M} \sum_{\ell \in [n_j(\bb)]} v_j(\ell) \le \sum_{j \in M} \sum_{\ell \in [n_j(\bb)]} v_j(1) \le \sum_{j \in M} n \cdot v_j(1) \le n \cdot m \cdot (\max_{j} v_j(1))$. As the game is an exact potential game, every $\epsilon$-better-response move increases the potential by more than $\epsilon$. So, in $n \cdot m \cdot (\max_{j} v_j(1)) / \epsilon$ steps the sequence should converge to an $\epsilon$-PNE.
\end{proof}

Corollary~\ref{thm:pseudoPolyBR} provides a pseudo-polynomial bound in the number of steps required for convergence to an approximate PNE, which can be meaningful in situations where the prizes (i.e., the values $v_j(1)$) are not very large. It also implies that an $\epsilon$-PNE can be computed in pseudo-polynomial time if we can compute $\epsilon$-better-responses efficiently.

\subsection{Social Welfare and Price of Anarchy}\label{sec:poa}
To start, let us briefly discuss what would be a natural definition(s) of social welfare for multi-activity games.

Consider first the budget model. From the perspective of the players, 
the social welfare naturally corresponds to the total prize allocated. 
This definition is also natural from the perspective of the contests.
Indeed, consider the motivating example involving the social media curators (players) and subscribers (contests). The welfare of the curators corresponds to the total subscribers' attention they receive, which is equal to the total prize allocated. On the other hand, the welfare of the subscribers corresponds to the compatible curators who serve them, which again corresponds to the total prize allocated. For this definition of social welfare, we prove a PoA bound of $2$, and this bound is tight (see Example 5.37 of \citet{vojnovic2015contest}).
% while the welfare of the subscribers is the amount of relevant  First, we can have the same definition that we had for the players: total prize allocated (which may correspond to the total satisfaction of the contests, consider the social media subscriber example). Second, we can maximize the total value of contests that are satisfied (won) by some player, assuming that multiple players satisfying the same contest does not add value.

For the cost model, the formulation of social welfare can be similarly motivated, with or without subtracting the cost. If one assumes that the cost to the players is a sunk cost, then it is reasonable to subtract it from the social welfare. On the other hand, if one assumes that the cost gets transferred to the contests (or the society), then it should not be subtracted. In any case, for both of these definitions, the PoA turns out to be infinite.

\subsubsection{Budget Model}
For the budget model, the social welfare is equal to the total prize that gets allocated: 
\begin{equation}\label{eq:SocialWelfareBud}
    \sw(\bb) = \sum_{i \in N} u_i(\bb) = \sum_{i \in N} v_j(n_j(\bb)) \cdot\b1\{i \in N_j(\bb)\} = \sum_{j \in M} v_j(n_j(\bb))\cdot n_j(\bb) .
\end{equation}
% The second definition, slightly less natural but may still be meaningful, corresponds to the total value of the contests that are won by at least one player. We assume that the value of a contest $j$ is $v_j(1)$. A loss in welfare occurs if some contests are not able to allocate their prize to any player.
% \begin{equation}
%     sw_2(\bb) = \sum_{j \in M} v_j(1) \b1\{n(\bb) > 0\}. \label{eq:swBudget2}
% \end{equation}
To prove the PoA bound of $2$ we shall use the result of \citet{vetta2002nash} for \textit{submodular} social welfare functions. Informally, this result states that the PoA bound of $2$ holds if the following conditions are satisfied:
\begin{enumerate}
    \item the utility of the players and the social welfare are measured in the same units,
    \item the total utility of the players is at most the social welfare,
    \item the social welfare function is non-decreasing and submodular, and
    \item the private utility of a player is at least as much as the \textit{Vickrey utility} (see equation~\eqref{eq:vickrey}).
\end{enumerate}
By definition, our model satisfies the first two requirements on this list. To show that it also satisfies the last two requirements, we reinterpret it using a different notation.

In the budget game, an action by a player $i$ effectively corresponds to a subset of the contests that $i$ wins. The output vector produced by the player to win a given set of contests is not important as long as the set of contests that she wins remains the same. Hence, we will represent the action taken by player $i$ as a subset of elements from a set of size $m$, as follows:
Let $\cG$ denote a set of $n \cdot m$ elements partitioned into $n$ size-$m$ sets $\cG^1, \cG^2, \ldots, \cG^n$, where $\cG^i = \{g^i_1, g^i_2, \ldots, g^i_m\}$. We represent the set of feasible actions for player $i$ by $\cA_i \subseteq 2^{\cG^i}$: an action $A_i \in\cA_i$
contains $g^i_j$ if and only if player $i$ satisfies the criteria for contest $j \in M$.
Note that $\emptyset \in \cA_i$, because we assume that each player is allowed to not participate and produce a $\bm{0}$ output (which does not win her any contests). An action profile $A = (A_i)_{i \in N} \in \times_{i \in N} \cA_i $ can be equivalently written as $\cup_{i \in N} A_i \in \cup_{i \in N} \cA_i$ because the sets $\cA_i$ are disjoint as per our notation.

As before, let $N_j(A) = \{ i \mid g^i_j \in A \}$ denote the players who win contest $j$ for action profile $A$, and let $n_j(A) = |N_j(A)|$.
The utility functions and the social welfare function can be rewritten using the new set notation as follows:
\begin{align*}
    u_i(A) &= \sum_{j \in M} v_j( n_j(A) ) \cdot \b1\{g^i_j \in A\},\\ % v_j( |\{ \iota \mid g^{\iota}_j \in A \}| ) \b1\{g^i_j \in A\},\\
    \sw(A) &= \sum_{i \in N} u_i(A) = \sum_{j \in M} v_j( n_j(A) ) \cdot n_j(A).
\end{align*}

Let us formally define submodular set functions.
% \begin{definition}
% A function $f: 2^{\cG} \rightarrow \bR$ is non-decreasing if: for $S, T \subseteq \cG$, $S \subseteq T$, $f$ satisfies $f(S) \le f(T)$.
% \end{definition}
\begin{definition}
A function $f: 2^{\Omega} \rightarrow \bR$ is {\em submodular} if 
for every pair of subsets $S, T \subseteq \Omega$ such that $S \subseteq T$
and every $x \in \Omega \setminus T$ we have
\[
    f(S \cup \{x\}) - f(S) \ge f(T \cup \{x\}) - f(T).
\]
\end{definition}

The next two lemmas prove that our model satisfies the conditions required to use the result of \citet{vetta2002nash}.
\begin{lemma}\label{thm:PoA:1}
For the budget model, if the total prize allocated by a contest is a weakly concave function of the number of winners of the contest, then the social welfare function is submodular.
\end{lemma}
\begin{proof}
Let $S, T \subseteq \cG$, $S \subseteq T$, and $x \in \cG \setminus T$. We need to show that 
\[
    \sw(S \cup \{x\}) - \sw(S) \ge \sw(T \cup \{x\}) - \sw(T).
\]
Let $x = g^i_j$ for some player $i$ and contest $j$. As $S \subseteq T$, $n_j(S) \le n_j(T)$. Now, as the total prize allocated by contest $j$ (which is equal to $\ell \cdot v_j(\ell)$ if there are $\ell$ winners) is a concave function, we get
\begin{align*}
    (n_j(S) + 1) \cdot v_j(n_j(S) + 1) - n_j(S) \cdot v_j(n_j(S)) \ge (n_j(T) + 1) \cdot v_j(n_j(T) + 1) - n_j(T) \cdot v_j(n_j(T)).
\end{align*}
As $n_{j}(S \cup \{x\}) = n_{j}(S) + 1$ and $n_{j}(T \cup \{x\}) = n_{j}(T) + 1$, and $n_{j'}(S \cup \{x\}) = n_{j'}(S)$ and $n_{j'}(T \cup \{x\}) = n_{j'}(T)$ for $j' \neq j$, we get the required result.
\end{proof}

The {\em Vickrey utility} of player $i$ 
at an action profile $A$ is the loss incurred by other players due to $i$'s participation, i.e., 
\begin{equation}\label{eq:vickrey}
    u_i^\text{Vickrey}(A) = \sum_{q \neq i} u_{q}(\emptyset, A_{-i}) - \sum_{q \neq i} u_{q}(A_i, A_{-i}),
\end{equation}
where $\emptyset$ is the action to not participate (or, equivalently, produce $0$ output and not win any contests).

\begin{lemma}\label{thm:PoA:2}
For the budget model, if the total prize allocated by a contest is a non-decreasing function of the number of winners of the contest, then 
for every profile $A$ and every player $i$, the utility of $i$ is at least as large as her Vickrey utility, i.e., 
    \[
        u_i(A_i, A_{-i}) \ge u_i^\text{Vickrey}(A).
    \]
\end{lemma}
\begin{proof}
By definition of $u_i$,
\begin{equation}\label{eq:prf:PoA:1}
    u_i(A_i, A_{-i}) = \sum_{j : g^i_j \in A_i} v_j( n_j(A_i, A_{-i}) ) = \sum_{j : g^i_j \in A_i} v_j( n_j(\emptyset, A_{-i}) + 1 ).
\end{equation}
By changing her action from $\emptyset$ to $A_i$, player $i$ starts winning contests in $J = \{j \mid g^i_j \in A_i\}$. Therefore, she affects the prize allocation of players who were already receiving prizes from contests in $J$. In particular, for any $j \in J$, the $n_j(\emptyset, A_{-i})$ players who were receiving a prize of $v_j( n_j(\emptyset, A_{-i}) )$ now receive a prize of $v_j( n_j(\emptyset, A_{-i}) + 1 )$. So,
\begin{equation}\label{eq:prf:PoA:2}
    \sum_{\iota \neq i} u_{\iota}(\emptyset, A_{-i}) - \sum_{\iota \neq i} u_{\iota}(A_i, A_{-i}) = \sum_{j \mid g^i_j \in A_i} n_j(\emptyset, A_{-i}) \cdot (v_j( n_j(\emptyset, A_{-i}) ) - v_j( n_j(\emptyset, A_{-i}) + 1 )).
\end{equation}
As the total prize allocated by a contest is a non-decreasing function of the number of winners, we have
\begin{align*}%\label{eq:prf:PoA:3}
     (n_j(\emptyset, A_{-i}) + 1) \cdot v_j( n_j(\emptyset, A_{-i}) + 1 ) &\ge n_j(\emptyset, A_{-i}) \cdot v_j( n_j(\emptyset, A_{-i}) ) \\
     \implies v_j( n_j(\emptyset, A_{-i}) + 1 ) &\ge n_j(\emptyset, A_{-i}) \cdot (v_j( n_j(\emptyset, A_{-i}) ) - v_j( n_j(\emptyset, A_{-i}) + 1 )) \\
     \implies \sum_{j : g^i_j \in A_i} v_j( n_j(\emptyset, A_{-i}) + 1 ) &\ge \sum_{j : g^i_j \in A_i} n_j(\emptyset, A_{-i}) \cdot (v_j( n_j(\emptyset, A_{-i}) ) - v_j( n_j(\emptyset, A_{-i}) + 1 )).
\end{align*}
Combining this inequality with \eqref{eq:prf:PoA:1} and \eqref{eq:prf:PoA:2}, we get the required result.
\end{proof}

\begin{theorem}\label{thm:swBudMul}
The social welfare in any mixed-strategy Nash equilibrium of a multi-activity budget game is at least $1/2$ of the optimum social welfare.
\end{theorem}
\begin{proof}
The social welfare is a non-decreasing function, as the total prize allocated by a contest weakly increases as the number of winners increases. This observation, together with Lemmas~\ref{thm:PoA:1} and~\ref{thm:PoA:2}, shows that our setting satisfies the necessary conditions of Theorem~5 of
\citet{vetta2002nash}. This gives us the required bound on the price of anarchy.
\end{proof}


\subsubsection{Cost Model}
As discussed before, we consider two definitions of social welfare for the cost model. The first definition does not subtract the costs from social welfare and corresponds to the definition given in \eqref{eq:SocialWelfareBud}. The second definition subtracts the costs from the social welfare and is equal to
\begin{equation}\label{eq:SocialWelfareCost}
    \overline{\sw}(\bb) = \sum_{i \in N} (u_i(\bb) - c_i(\bb)) = \sum_{i \in N} (v_j(n_j(\bb)) \cdot\b1\{i \in N_j(\bb)\} - c_i(\bb)) = \sum_{j \in M} v_j(n_j(\bb)) \cdot n_j(\bb) - \sum_{i \in N} c_i(\bb).
\end{equation}
Next, we prove that the PoA can be unbounded for both definitions of social welfare in the cost model.
\begin{theorem}\label{thm:swCost}
The social welfare in a pure-strategy Nash equilibrium of a multi-activity cost game can be arbitrarily low compared to the optimum social welfare.
This holds even if there are at most two players, two activities, and two contests.
\end{theorem}
\begin{proof} We analyze the two variants of the model separately.

\smallskip

\noindent\textbf{Subtracting Costs from Social Welfare.}
We will construct an instance with two players, two activities, and two contests, i.e., $n=k=m=2$. Contest $j$ distributes a prize of $1$ to players who produce an output of $1$ along activity $j$ and does not care about the output along activity $(3-j)$. Player $i$ has a cost of $(1/2 + \epsilon)$ for producing an output of $1$ along activity $i$, and a cost of $(1-\epsilon)$ for producing an output of $1$ along activity $(3-i)$.

Consider the following PNE: player $i$ is producing an output of $1$ along activity $(3-i)$ and an output of $0$ along activity $i$; therefore, each player has a cost of $(1-\epsilon)$, a prize of $1$, and a utility of $\epsilon$. Notice that this is a PNE because if any player $i$ decides to produce output along activity $i$ (which they are currently not doing), then they will get an additional prize of $1/2$ for a cost of $(1/2 + \epsilon)$, which decreases their utility. The total welfare for this equilibrium is $2 (1 - (1-\epsilon)) = 2\epsilon$.

Consider the socially optimal situation where each player $i$ produces output along activity $i$: the total prize allocation is still $2$, but the total cost is $2(1/2+\epsilon)$, so the total welfare is $(1-2\epsilon)$. Therefore, the price of anarchy is $\frac{1-2\epsilon}{2\epsilon}$, which tends to $+\infty$ as $\epsilon \rightarrow 0$.

\smallskip

\noindent\textbf{Not Subtracting Costs from Social Welfare.} In this definition of social welfare, too, a simple example shows that the price of anarchy is unbounded. Consider an instance with one player, two activities, and two contests. The two activities have a one-to-one correspondence with the contests, i.e., contest $j$ cares only about activity $j$. The player can win the first contest, which has a prize of $\epsilon$, with a cost of $\epsilon/2$, and she can win the second contest, which has a prize of $1$, with a cost of $1$. In equilibrium, the player only wins the first contest. The price of anarchy is $1/\epsilon$, which tends to $+\infty$ as $\epsilon \rightarrow 0$. 
Here, the social welfare and the utility of the player are not aligned, as the player cares about costs whereas the social welfare does not. Hence a bad PoA is expected.
\end{proof}


==> ec/ppad-pls.tex <==
\section{Single-Activity: PPAD$\cap$PLS-Completeness }\label{sec:singleActivity}

% In this model, where a player can produce output along multiple activities simultaneously, we shall prove that it is NP-hard for a player to best respond to the strategies of other players. This implies hardness for finding an equilibrium. We also prove a similar result for the multi-activity cost model.

% Noting the hardness result, we consider a restricted setup where the players can produce output along a set of portfolios of activities. A player selects a portfolio $p$ from the set of portfolios $\cP_i \subset \bR_{\ge 0}^k$ and produces output proportional to $p$. We assume that the set of portfolios is finite and of polynomial size. 

% This portfolio model can easily be reduced to a model where a player $i$ can produce output along only one activity, where an activity in this model corresponds to a portfolio in the previous model; we call this the \textit{single-activity} model. In the single-activity budget model, $\cB_i$ is associated with a vector $\bar{\bb}_i \in \bR_{\ge 0}^k$ of upper-limits; for any $b_i \in \cB_i$, there is an activity $\ell \in K$ such that $0 \le b_{i,\ell} \le \bar{b}_{i,\ell}$ and $b_{i,t} = 0$ for all $t \neq \ell$. Although the feasible set of outputs $\cB_i$ is not convex in the single-activity budget model, in Lemma~\ref{thm:sin2mulBudRed}, we shall prove that it can be reduced to the multi-activity budget model, and therefore, all positive results for the multi-activity budget model apply to this model. We shall also prove similar positive results for the cost model, both single-activity and multi-activity.

% For the single-activity models, both budget and cost, best-response is easy for a player. But, here we will prove a PLS-completeness result for finding a PNE and (PPAD$\cap$PLS)-completeness result for finding an MNE.

% In the previous section, we saw that it is NP-hard for the players to best respond to the strategies of other players, and so it is NP-hard to find a PNE for the multi-activity cost and budget games. 
In this section, we focus our attention on the single-activity model and show that, for both cost and budget models, it is PLS-complete to find a pure Nash equilibrium and (PPAD$\cap$PLS)-complete to find a mixed Nash equilibrium (MNE). Note that the set of MNEs of a game is a super-set of the set of PNEs, so finding an MNE is at least as easy as finding a PNE.

In a single-activity game, for every player $i$, there is at most one activity $\ell$ for which the output $b_{i,\ell}$ may be strictly greater than $0$; for every other activity $\ell' \neq \ell$, $b_{i,\ell'} = 0$. Additionally, 
we assume that each contest $i$ has a fixed total prize, 
which it distributes equally among all winners.

\begin{theorem}\label{thm:ppadPls}
In the single-activity models, both cost and budget, it is ({\sc PPAD}\,$\cap$\,{\sc PLS})-complete to find a mixed-strategy Nash equilibrium. 
\end{theorem}
A recent paper by \citet{fearnley2021complexity} proved the interesting result that finding a fixed-point of a $2$-dimensional smooth function ($f : [0,1]^2 \rightarrow \bR$) given by a circuit of addition and multiplication operators using gradient descent, {\sc 2D-GD-FixedPoint}, is complete for the class PPAD$\cap$PLS. Based on this result, \citet{babichenko2021settling} proved that the problem of computing an MNE of an explicit congestion game, {\sc ExpCong}, is also complete for PPAD$\cap$PLS. \citet{babichenko2021settling} do this by first reducing {\sc 2D-GD-FixedPoint} to identical interest 5-polytensor games, {\sc 5-Polytensor}, and then {\sc 5-Polytensor} to {\sc ExpCong}. In our proof for Theorem~\ref{thm:ppadPls}, we reduce {\sc 5-Polytensor} to the single-activity game, proving the required result.

Before moving to the proof, let us define identical interest polytensor games, {\sc $\kappa$-Polytensor}. Polytensor games are a generalization of the better known polymatrix games, {\sc Polymatrix}; {\sc Polymatrix} = {\sc $2$-Polytensor}.
\begin{definition}[{\sc Polymatrix}: Identical Interest Polymatrix Game]
There are $n$ players. Player $i$ chooses from a finite set of actions $A_i$. The utility of player $i$ for action profile $(a_i, \ba_{-i}) = \ba = (a_j)_{j \in [n]} \in \times_{j \in [n]} A_j$ is given by $u_i(\ba) = \sum_{j \in [n], j \neq i} u_{i,j}(a_i, a_j)$, where $u_{i,j} : A_i \times A_j \rightarrow \bR_{\ge 0}$. The players have identical interest, i.e., $u_{i,j} = u_{j,i}$.
\end{definition}
The definition of {\sc $\kappa$-Polytensor} is similar to {\sc Polymatrix}, instead of $u_{i,j}$ we have $u_S$ where $S \subseteq [n], |S| = \kappa$.
\begin{definition}[{\sc $\kappa$-Polytensor}: Identical Interest $\kappa$-Polytensor Game]\label{def:polytensor}
There are $n$ players. Player $i$ chooses from a finite set of actions $A_i$. 
The utility of player $i$ for action profile $\ba = (a_j)_{j \in [n]} \in \times_{j \in [n]} A_j$ is given by $u_i(\ba) = \sum_{S \subseteq [n], i \in S, |S| = \kappa} u_S(\ba_S)$, where $\ba_S = (a_j)_{j \in S}$ is the action profile of the players in $S$ and $u_S : \times_{j \in S} A_j \rightarrow \bR_{\ge 0}$.
\end{definition}
When the number of actions for each player, $|A_i|$, is bounded by $m$, note that the representation size of a {\sc $\kappa$-Polytensor} game is $O(n^{\kappa}m^{\kappa})$. In particular, if $\kappa$ is a constant and
$m = poly(n)$, then {\sc $\kappa$-Polytensor} games admit a succinct representation.

\begin{proof}[Proof of Theorem~\ref{thm:ppadPls}]
Let us first focus on the single-activity budget model, towards the end we shall extend this to the cost model. Below, we provide a reduction from {\sc $3$-Polytensor} for a cleaner presentation of the main steps. Similar steps with more calculations apply to {\sc $5$-Polytensor}, provided in the appendix.

\textbf{Budget.} Take an arbitrary instance of {\sc $3$-Polytensor} with $n$ players; we shall use the same notation as Definition~\ref{def:polytensor}. We construct a single-activity game with $n$ players, $\sum_{i \in [n]} |A_i|$ activities, and a polynomial number of contests to be defined later.

The $\sum_{i \in [n]} |A_i|$ activities have a one-to-one association with the actions of the players. The activities are partitioned into $n$ subsets; the $i$-th subset has size $|A_i|$ and is associated with player $i$; we identify these activities by $A_i$. Player $i$ has a budget of $1$ that they can use to produce output along any activity from $A_i$, but they have $0$ budget for the activities in $A_j$ for $j \neq i$. Effectively, as we are in a single-activity model, player $i$ selects an activity from the activities in $A_i$ and produces an output of $1$ along it. Note that the players have disjoint sets of activities for which they can produce outputs.

All the contests we construct are associated with exactly three players and at most three activities. We shall denote a contest by $\cC_{i,j,k}(A)$, where
\begin{itemize}
    \item $i$, $j$, and $k$ are the three distinct players based on whose utility function in the polytensor game, $u_{i,j,k}$, we shall specify the prize of contest $\cC_{i,j,k}(A)$;
    \item the contest $\cC_{i,j,k}(A)$ awards its prize to any player who produces an output of at least $1$ along the activities in $A$;
    \item the activities in $A$ are from $A_i \cup A_j \cup A_k$ with $|A| \le 3$ and $ |A \cap A_{\ell}| \le 1$ for $\ell \in \{i,j,k\}$.
\end{itemize}
We shall call a contest $\cC_{i,j,k}(A)$ a Type-$\ell$ contest if $|A| = \ell$.

Let us focus on a fixed set of three players $\{i,j,k\}$. We create contests to exactly replicate the utility that these players get from $u_{i,j,k}$. If we can do this, then repeating the same process for every set of three players, we will replicate the entire {\sc $3$-Polytensor} game. The utility that player $i$ gets from $u_{i,j,k}$ is $u_{i,j,k}(a_i,a_j,a_k)$, where the $a_i,a_j,a_k$ are the actions of the three players.
We have the following contests:

% \begin{enumerate}
    % \item 
\textbf{Type-3 Contests.} Let us add a contest $\cC_{i,j,k}(a_i,a_j,a_k)$ with prize $v_{i,j,k}(a_i,a_j,a_k)$ for every $(a_i,a_j,a_k) \in A_i \times A_j \times A_k$. We shall specify the $v_{i,j,k}(a_i,a_j,a_k)$ values based on $u_{i,j,k}(a_i,a_j,a_k)$ values, later. Contest $\cC_{i,j,k}(a_i,a_j,a_k)$ distributes a prize of $v_{i,j,k}(a_i,a_j,a_k)$ to players who produce output along the activities $a_i$, $a_j$, or $a_k$. 
    
Say the players $i,j,k$ play the actions $a_i^*, a_j^*, a_k^*$. 
% Let $A_j^- = A_j \setminus \{a_j^*\}$; and for $T \subseteq S$, let $A_T^- = \times_{j \in T} A_j^-$. 
The total prize that player $i$ gets from the contests we added is:
\begin{align}\label{eq:ppadPls:1}
    &\frac{1}{3}{v_{i,j,k}(a_i^*,a_j^*,a_k^*)}
    + \sum_{a_j \neq a_j^*} \frac{1}{2}{v_{i,j,k}(a_i^*,a_j,a_k^*)}  + \sum_{a_k \neq a_k^*} \frac{1}{2}{v_{i,j,k}(a_i^*,a_j^*,a_k)}
    + \sum_{\substack{a_j \neq a_j^* \\ a_k \neq a_k^*}} v_{i,j,k}(a_i^*,a_j,a_k).
\end{align}
In the above expression, the first term is for the prize that $i$ shares with $j$ and $k$, the second term is for the prizes that $i$ share with only $k$ but not $j$, similarly, the third term is for the prizes that $i$ shares only with $j$ but not $k$, and the fourth term is for the prizes it does not share with $j$ or $k$. 

In the above expression, the first term $\frac{1}{3}{v_{i,j,k}(a_i^*,a_j^*,a_k^*)}$ resembles the utility  that the players get in the polytensor game, $u_{i,j,k}(a_i^*,a_j^*,a_k^*)$. If we were to set $v_{i,j,k}(a_i^*,a_j^*,a_k^*) = 3 u_{i,j,k}(a_i^*,a_j^*,a_k^*)$, then it will exactly be equal. But, unless we take care of the additional terms in the expression, we are not done. We shall add Type-1 and Type-2 contests to cancel the additional terms.

The expression in \eqref{eq:ppadPls:1} can be rewritten as
\begin{align*}
    &\sum_{a_j \in A_j, a_k \in A_k} v_{i,j,k}(a_i^*,a_j,a_k) - \sum_{a_j \neq a_j^*} \frac{1}{2}{v_{i,j,k}(a_i^*,a_j,a_k^*)} - \sum_{a_k \neq a_k^*} \frac{1}{2}{v_{i,j,k}(a_i^*,a_j^*,a_k)}
    -\frac{2}{3}{v_{i,j,k}(a_i^*,a_j^*,a_k^*)}.
\end{align*}

\textbf{Type-1 Contests.} Let us add a contest $\cC_{i,j,k}(a_i')$ with prize $\sum_{a_i \neq a_i', a_j \in A_j, a_k \in A_k} v_{i,j,k}(a_i,a_j,a_k)$ for every $a_i' \in A_i$. This contest $\cC_{i,j,k}(a_i')$ awards its prize to any player who produces output along activity $a_i'$ (effectively it awards the prize to player $i$ if they produce output along $a_i'$, because no other player can produce output along $a_i'$). Similarly, we add the contests $\cC_{i,j,k}(a_j')$ and $\cC_{i,j,k}(a_k')$ for $a_j' \in A_j$ and $a_k' \in A_k$, respectively. The total prize that player $i$ gets from Type-1 and Type-3 contests is
\begin{align*}
    &\sum_{a_i,a_j,a_k} v_{i,j,k}(a_i,a_j,a_k) - \sum_{a_j \neq a_j^*} \frac{1}{2}{v_{i,j,k}(a_i^*,a_j,a_k^*)} - \sum_{a_k \neq a_k^*} \frac{1}{2}{v_{i,j,k}(a_i^*,a_j^*,a_k)}
    -\frac{2}{3}{v_{i,j,k}(a_i^*,a_j^*,a_k^*)}.
\end{align*}
As $\sum_{a_i,a_j,a_k} v_{i,j,k}(a_i,a_j,a_k)$ does not depend upon the action $a_i^*$ selected by $i$, the utility of player $i$ is effectively
\begin{equation*}
    - \sum_{a_j \neq a_j^*} \frac{1}{2}{v_{i,j,k}(a_i^*,a_j,a_k^*)} - \sum_{a_k \neq a_k^*} \frac{1}{2}{v_{i,j,k}(a_i^*,a_j^*,a_k)} -\frac{2}{3}{v_{i,j,k}(a_i^*,a_j^*,a_k^*)}.
\end{equation*}

\textbf{Type-2 Contests.} Let us add a contest $\cC_{i,j,k}(a_i', a_j')$ with prize $\sum_{a_k \in A_k} \frac{1}{2}{v_{i,j,k}(a_i',a_j',a_k)}$ for every $a_i' \in A_i$ and $a_j' \in A_j$. This contest $\cC_{i,j,k}(a_i', a_j')$ awards its prize to players who produce output along activity $a_i'$ or $a_j'$. In a similar manner, we add contests corresponding to the actions of the other $5$ possible combinations of players among the three players $i,j,k$, like $\cC_{i,j,k}(a_i', a_k')$ for $a_i' \in A_i$ and $a_k' \in A_k$, and so on. The net utility that player $i$ gets from Type-1, Type-2 and Type-3 contests is
\begin{equation*}
    \frac{1}{3}{v_{i,j,k}(a_i^*,a_j^*,a_k^*)}.
\end{equation*}
We set $v_{i,j,k}(a_i,a_j,a_k) = 3 u_{i,j,k}(a_i,a_j,a_k)$ for every $(a_i, a_j, a_k) \in A_i \times A_j \times A_k$, and we are done.

\textbf{Cost.} It is easy to adapt the above proof to the single-activity cost model. All the players, contests, and activities are the same, we just need to replace the budgets with costs. In the proof above, we used the budgets to make sure that player $i$ can produce output only along activities in $A_i$. We can achieve that same for the cost model: for player $i$, set a very low cost for the activities in $A_i$ and very high cost for the activities in $A_j$, $j \neq i$, such that player $i$ always wants to produce output along the activities in $A_i$ and never along the activities not in $A_i$.
\end{proof}

In the previous theorem, we analyzed the complexity of computing an MNE. As we have shown earlier, single-activity cost and budget games always have a PNE, and therefore, it is relevant to know the complexity of computing a PNE. 
% Note that computing a PNE is at least as hard as computing an MNE, because a PNE is also an MNE. 
In the next theorem, we prove that computing a PNE is PLS-complete, and this is true even if all the players are identical. In the proof, we reduce {\sc Max-Cut} to the problem of finding a PNE in a particular class of single-activity games with identical players. For this class of single-activity games, finding an MNE is easy, which highlights that the class of single-activity games where PNE is hard (PLS-complete) to compute is strictly larger than the class of single-activity games where MNE is hard (PPAD$\cap$PLS-complete) to compute. % The proof is provided in the appendix.
\begin{theorem}\label{thm:plsCompleteness}
In the single-activity models, both cost and budget, it is {\em PLS}-complete to find a pure-strategy Nash equilibrium. The result holds even if all players are identical.
\end{theorem}
\begin{proof} %[Proof of Theorem~\ref{thm:plsCompleteness}]
We prove this result by reducing the problem of finding a locally optimal max-cut solution in a graph, which is known to be a PLS-complete problem~\cite{johnson1988easy}, to our problem. Let $(V,E)$ be an arbitrary graph and let $w_e \in \bZ_{\ge 0}$ be the weight of edge $e \in E$. A cut $(S,\overline{S})$ (where $\overline{S} = V \setminus S$) is locally optimal if one cannot improve the max-cut objective $\sum_{(u,v) \in E, u \in S, v \in \overline{S}} w_{u,v}$ by moving a vertex $u$ from its current partition $S$ (or $\overline{S}$) to the other partition $\overline{S}$ (or $S$). 

\textbf{Budget.} Let us first focus on the single-activity budget model, we shall slightly tweak the same construction for the single-activity cost model.

\textit{Construction.} We construct an instance of the budget game corresponding to the given graph $(V,E)$ as follows:
\begin{enumerate}
    \item Let there be $|V|$ players.
    \item Let there be $2|V|$ activities, which we identify by $\alpha_v$ and $\beta_v$ for $v \in V$.
    \item Let each player have a budget of $1$ that they can spend on any of the activities. As we are in a single-activity setup, in a pure strategy, a player would select an activity and produce an output of $1$ along that activity. Note that the strategy space is symmetric across the players.
    \item Let there be $|V| + 2|E|$ contests. 
    \begin{itemize}
        \item We identify the first $|V|$ contests using the vertices. The contest that corresponds to $v \in V$ equally distributes a large prize of $4\sum_{e \in E} w_e + 2$ to the players who produce a total output of at least $1$ along the two activities $\alpha_v$ and $\beta_v$ corresponding to $v$, i.e., a player $i$ receives a share of the prize if $b_{i,\alpha_v} + b_{i,\beta_v} \ge 1$. We call these contests \textit{vertex} contests.
        \item We identify the other $2|E|$ contests using the edges, two contests per edge. For an edge $e = (u,v) \in E$, one of the contests distributes a prize of $w_e$ to the players who produce an output of at least $1$ along the two activities $\alpha_u$ and $\alpha_v$, and the other contest distributes a prize of same value $w_e$ to the players who produce an output of at least $1$ along $\beta_u$ and $\beta_v$. We call these contests \textit{edge} contests.
    \end{itemize}
\end{enumerate}

\textit{Analysis.} Observe that the total prize awarded by the $2|E|$ edge contests is $2(\sum_{e \in E} w_e)$, while the prize awarded by a single vertex contest is $4\sum_{e \in E} w_e + 2$, which is much larger. As a player can produce output along only one activity, and as each vertex contest $v$ values a unique disjoint pair of activities $(\alpha_v, \beta_v)$, no player can win prizes from more than one vertex contest. Also, as the number of players is equal to the number of the vertex contests, each player can get a complete share of one of the vertex contests. In a PNE, each player selects a distinct pair $(\alpha_v, \beta_v)$ and produces output along one of the activities in the pair, because a player can move from a shared prize to an unshared prize increasing their utility by at least $2\sum_{e \in E} w_e + 1$ from the vertex contests, which dominates maximum total loss of $2\sum_{e \in E} w_e$ from the $2|E|$ edge contests. Let us denote the player who produces output along the pair of activities $(\alpha_v, \beta_v)$ as $i_v$.

Let $S = \{ v \in V \mid b_{i_v,\alpha_v} = 1 \}$ and $\overline{S} = V \setminus S = \{ v \in V \mid b_{i_v,\beta_v} = 1 \}$. For an edge $(u,v)$, if both players $i_u$ and $i_v$ are in $S$ or $\overline{S}$, then they share the prize of $w_{u,v}$, on the other hand if one of them is in $S$ and the other in $\overline{S}$ then they each get $w_{u,v}$. The value of the potential function (Equation~\eqref{eq:potFun}) $\phi$ can be written using $S$ and $\overline{S}$ as
\begin{multline*}
    \phi(S,\overline{S}) = \left(4\sum_{e \in E} w_e + 2\right) |V| + \left( \frac{3}{2} \sum_{e \in E} w_e + \frac{1}{2} \sum_{(u,v) \in E, u \in S, v \in \overline{S}} w_{u,v} \right) \\
    = \left(4 |V| + \frac{3}{2} \right) \sum_{e \in E} w_e + 2 |V| + \frac{1}{2}\sum_{(u,v) \in E, u \in S, v \in \overline{S}} w_{u,v},
\end{multline*}
where the contribution of $|V| (4\sum_{e \in E} w_e + 2)$ is from the $|V|$ vertex contests and a contribution of $3 w_{u,v}/2$ (if both $u$ and $v$ are in $S$ or $\overline{S}$) or $2 w_{u,v}$ (if one of $u$ or $v$ is in $S$ and the other in $\overline{S}$) is from the two contests corresponding to the edge $(u,v)$. As we have argued before, a player $i_v$ will never change their associated vertex $v$ in a better response move. A move by the player $i_v$ of shifting from $\alpha_v$ to $\beta_v$, or vice-versa, corresponds to moving the vertex $v$ across the cut $(S, \overline{S})$ in the max-cut problem. The value of the potential is effectively equal to the objective of the max-cut problem: we have multiplied the max-cut objective with a positive constant factor of $1/2$ and added a constant term. So, we have a one-one correspondence between local search in max-cut and dynamics in the single-activity budget game.

\textbf{Cost.} Note that for the budget game constructed above, the budget constraint was not very crucial in the analysis. No player had an incentive to produce an output of strictly more than $1$ along the activity they selected, because all the contests already awarded the prizes as soon as the players produced an output of $1$. In the cost model, we remove the budget constraint and set $c_{i, \ell} = 4\sum_{e \in E} w_e + 2$ for every player $i$ and activity $\ell$. The same analysis used in the budget model holds here too, the value of the potential function (Equation~\eqref{eq:potFun}) here is:
\begin{multline*}
    \phi(S,\overline{S}) = \left(4\sum_{e \in E} w_e + 2\right) |V| + \left( \frac{3}{2} \sum_{e \in E} w_e + \frac{1}{2} \sum_{(u,v) \in E, u \in S, v \in \overline{S}} w_{u,v} \right) - \left(4\sum_{e \in E} w_e + 2\right) |V| \\
    = \frac{3}{2} \sum_{e \in E} w_e + \frac{1}{2} \sum_{(u,v) \in E, u \in S, v \in \overline{S}} w_{u,v},
\end{multline*}
where the positive contribution of $|V| (4\sum_{e \in E} w_e + 2)$ is from the $|V|$ vertex contests, the contribution of $3 w_{u,v}/2$ or $2 w_{u,v}$ is from the two contests corresponding to the edge $(u,v)$, and a negative contribution of $|V| (4\sum_{e \in E} w_e + 2)$ is due to the cost of the players. The rest of the argument follows as before.

\textbf{Mixed-strategy Nash equilibrium.} In the {\sc Max Cut} problem, a randomized solution where each vertex is on either side of the cut with a probability of $1/2$ cannot be improved by moving just one vertex to a different side (or to a different distribution over the two sides). So, it is locally stable. We apply the same idea to find an MNE in the single-activity contest game just constructed.

Consider the following mixed strategy profile: for every $v \in V$, there is a unique player $i_v$ who produces an output of $1$ along one of the two activities $\alpha_v$ or $\beta_v$ with a probability of $1/2$ each. As argued before, player $i_v$ would not want to produce output along any other $\alpha_{u}$ or $\beta_u$ for $u \neq v$ because of the vertex contests. Also, given that every other player is following this strategy, player $i_v$ has the same utility for selecting either $\alpha_v$ or $\beta_v$, so $(1/2, 1/2)$ is as good a mixed-strategy as any other. So, we have an equilibrium.
\end{proof}


A direct corollary of this PLS-completeness result is that better/best-response dynamics takes an exponential number of steps to converge for some instances of the problem.

% A corollary of the PLS-completeness result is that for some instances of the game, better/best-response dynamics takes an exponential number of steps to converge to a PNE. This leads to a natural question: if we assume that a player only makes a move if it increases their utility by at least $\epsilon$, for some constant $\epsilon > 0$, does this process converge to an $\epsilon$-PNE in steps polynomial in $1/\epsilon$ and size of the problem? The answer to this question is negative for exact potential games in general~\cite{skopalik2008inapproximability}. Note that all PLS-complete problems have fully polynomial-time approximation schemes (FPTAS) with respect to the potential function~\cite{orlin2004approximate}, but approximation of the potential doesn't imply approximation of each player's utility, there may be a player who can make a move to significantly increase their utility as shown by~\cite{skopalik2008inapproximability}.

==> old/hardness.tex <==
\section{Analysis}
% The positive results mentioned above indicate that in these contests with equal sharing allocation a PNE exists and all PNEs have good social welfare. But a natural question arises, whether such a PNE is easy to compute and is efficiently reachable by the players? We answer this question negatively by showing: (1) it is NP-hard for a player to compute a strategic deviation (a.k.a. better/best response dynamics); (2) even with an exact oracle for better/best response, the dynamics may take exponential time to converge because this problem is PLS-complete, i.e., as hard as any local search problem~\cite{johnson1988easy}.
We now focus on the convex model and give the following hardness result.
\begin{theorem}
The problem of computing a best response to a given strategy of other players is NP-hard for the convex model. % \abheek{TODO: better response?}
\end{theorem}
\begin{proof}
This result can be shown by a reduction from the knapsack problem, even when there is only one player (i.e., no competition). Take an instance of knapsack with $n$ items with weights $w_1, \ldots, w_n$ and a total weight of $W$. The contest problem is defined as follows:

There are $n$ contests and $n$ activities. The contest $j$ has a prize of $w_j$. For contest $j$ and activity $k$, the function $f_{j,k}(x)$ is defined as:
\[
    f_{j,k}(x) = \begin{cases} 0, &\text{ if $j \neq k$} \\
    x/w_j, &\text{ if $j = k$} \end{cases}.
\]
The player has total budget of $W$ and can invest this budget in any of the activities. From the construction, it can be observed that the player needs to produce an output of $w_j$ along activity $j$ to have $f_{j,j}(w_j) \ge 1$ and win the contest $j$ with a prize $w_j$. With an output less than $w_j$ along activity $j$, the player doesn't get anything for this investment. So, effectively, the player needs to select a subset of activities $S$, and for every $j \in S$ it needs to produce an output of $w_j$, with $\sum_{j \in S} w_j$ less than or equal to the total budget $W$. From the last statement, it should be clear that this is the same optimization problem as the knapsack problem.
\end{proof}
Given this hardness result for the convex model, let us now focus on the single-activity model. We shall prove a PLS-completeness result for finding a PNE for the single-activity model, which automatically applies to the convex model. We shall use the following potential function to derive the PLS-completeness result. Note that this potential function can also be used to derive the PNE existence result of \cite{may2014filter,vojnovic2015contest}.

\paragraph{Potential Function.} A potential function for the game of simultaneous contest is
\begin{equation}\label{eq:equalSharingPotentialFunc}
    \phi(\bb) = \sum_{j \in M} w_j H(n_j(\bb)),
\end{equation}
where $H(p) = \sum_{\ell = 1}^p 1/\ell$ is the harmonic sum. This potential function can be derived using the path independence property of an exact potential game.

\begin{theorem}\label{thm:eqShr3}
The problem of finding a pure-strategy Nash equilibrium in the single-activity model (and therefore, the convex model) is PLS-complete, even if all players have the same strategy space.
\end{theorem}

\begin{proof}[Proof of Theorem~\ref{thm:eqShr3}]
We prove this result by reducing the problem of finding a locally optimal max-cut solution in a graph, which is known to be a PLS-complete problem~\cite{johnson1988easy}, to our problem. Let $(V,E)$ be an arbitrary graph and let $w_e$ be the weight of edge $e \in E$. A cut $(S,\overline{S})$ (where $\overline{S} = V \setminus S$) is locally optimal if one cannot improve the max-cut objective $\sum_{(u,v) \in E, u \in S, v \in \overline{S}} w_{u,v}$ by moving a vertex $u$ from its current partition $S$ (or $\overline{S}$) to the other partition $\overline{S}$ (or $S$). 

\textit{Construction.} We construct an instance of the simultaneous contest corresponding to the given graph $(V,E)$ as follows:
\begin{enumerate}
    \item There are $|V|$ players.
    \item There are $2|V|$ activities, which we will identify by $\alpha_v$ and $\beta_v$ for $v \in V$.
    \item Each player has a budget of $1$ that they can spend on any of the activities, i.e., $\cB_i = \{ \bb_i \in \bR^{2|V|} \mid \sum_{v \in V} b_{i,\alpha_v} + \sum_{v \in V} b_{i,\beta_v} \le 1 \}$. Note that the strategy space is symmetric across the players. \abheek{This is a slightly less restricted strategy space for the players compared to the single-activity case (convex combinations are being allowed). But this doesn't cause any issue with the proof, the players anyway will select one activity at a time. It may simplify it a bit. Update the proof at some point to remove this confusion. }
    \item There are $|V| + 2|E|$ contests. 
    \begin{itemize}
        \item We identify the first $|V|$ contests using the vertices. The contest that corresponds to $v \in V$ equally distributes a large prize of $4\sum_{e \in E} w_e + 2$ to the players who put an effort of at least $1$ in the two activities $\alpha_v$ and $\beta_v$ corresponding to $v$, i.e., a player $i$ receives a share of the prize if $b_{i,\alpha_v} + b_{i,\beta_v} \ge 1$. We call these contests \textit{vertex} contests.
        \item We identify the other $2|E|$ contests using the edges, two contests per edge. For an edge $e = (u,v) \in E$, one of the contests distributes a prize of $w_e$ to the players who put an effort of at least $1$ in the two activities $\alpha_u$ and $\alpha_v$, and the other contest awards a same prize of $w_e$ to the players who put an effort of at least $1$ in $\beta_u$ and $\beta_v$. We call these contests \textit{edge} contests.
    \end{itemize}
\end{enumerate}

\textit{Analysis.} Observe that the total prize awarded by the $2|E|$ contests corresponding to the edges is $2(\sum_{e \in E} w_e)$, while the prize awarded by a single contest corresponding to the vertices is $4\sum_{e \in E} w_e + 2$, which is much larger. As a player has a total budget of $1$ and needs to invest an effort of $1$ among the two activities $\alpha_v$ and $\beta_v$ to get (a share of) the prize given the vertex $v$ contest, it is a dominating strategy for the player to invest their entire budget to $\alpha_v$ and $\beta_v$ for some $v \in V$. Moreover, no two players select the same $v$ (pair $\alpha_v$ and $\beta_v$) to invest their efforts, because there are $|V|$ such contests, one for each player, and a player can move from a shared prize to a unshared prize increasing their utility by at least $2\sum_{e \in E} w_e + 1$, which dominates maximum total loss associated with the $2|E|$ edge contests. So, w.l.o.g. we assume that each player selects a distinct pairs ($\alpha_v$,$\beta_v$) to invest all their effort; we denote this player by $i_v$. 

Further, we can assume that the player $i_v$ invests all their effort to only one of $\alpha_v$ or $\beta_v$, because distributing their effort among the two activities doesn't give them any of the prizes awarded by the edge contests and don't have any effect on their prize from the vertex contests. Let $S = \{ v \in V \mid b_{i_v,\alpha_v} = 1 \}$ and $\overline{S} = V \setminus S = \{ v \in V \mid b_{i_v,\beta_v} = 1 \}$. For an edge $(u,v)$, is both players $i_u$ and $i_v$ are in $S$ or $\overline{S}$, then they share the prize of $w_{u,v}$, on the other hand if one of them is in $S$ and the other in $\overline{S}$ then they each get $w_{u,v}$. The value of the potential function $\phi$ can be written using $S$ and $\overline{S}$ as
\[ \phi(S,\overline{S}) = \Bigl(4 |V| + \frac{3}{2}\Bigr)\sum_{e \in E} w_e + 2 |V| + \frac{1}{2}\sum_{(u,v) \in E, u \in S, v \in \overline{S}} w_{u,v}, \]
where the contribution of $|V| (4\sum_{e \in E} w_e + 2)$ is from the $|V|$ vertex contests and a contribution of $3 w_{u,v}/2$ (if both $u$ and $v$ are in $S$ or $\overline{S}$) or $2 w_{u,v}$ (if one of $u$ or $v$ is in $S$ and the other in $\overline{S}$) from the two contests corresponding to the edge $(u,v)$. As we have argued above, a player $i_v$ will never change their associated vertex $v$ in a better response move. A move by the player $i_v$ of shifting effort from $\alpha_v$ to $\beta_v$, or vice-versa, corresponds to moving the vertex $v$ across the cut $(S, \overline{S})$ in the max-cut problem. So, we have a one-one correspondence between local search in max-cut and dynamics in the game of simultaneous contest.
\end{proof}

A corollary of the PLS-completeness result in Theorem~\ref{thm:eqShr3} is that for some instances of the game, a better/best-response dynamics takes an exponential number of steps to converge to a PNE. This leads to a natural question: if we assume that a player only makes a move if it increases their utility by at least $\epsilon$, for some constant $\epsilon > 0$, does this process converge to an $\epsilon$-PNE in steps polynomial in $1/\epsilon$ and size of the problem? The answer to this question is negative for exact potential games in general~\cite{skopalik2008inapproximability}. Note that all PLS-complete problems have fully polynomial time approximation schemes (FPTAS) with respect to the potential function~\cite{orlin2004approximate}, but approximation of the potential doesn't imply approximation of each player's utility, there may be a player who can make a move to significantly increase their utility as shown by~\cite{skopalik2008inapproximability}.
